Generalizing DP-SGD with Shuffling and Batch Clipping

Classical differential private DP-SGD implements individual clipping with random subsampling, which forces a mini-batch SGD approach. We provide a general differential private algorithmic framework that goes beyond DP-SGD and allows any possible first order optimizers (e.g., classical SGD and momentum based SGD approaches) in combination with batch clipping, which clips an aggregate of computed gradients rather than summing clipped gradients (as is done in individual clipping). The framework also admits sampling techniques beyond random subsampling such as shuffling. Our DP analysis follows the $f$-DP approach and introduces a new proof technique which allows us to derive simple closed form expressions and to also analyse group privacy. In particular, for $E$ epochs work and groups of size $g$, we show a $\sqrt{g E}$ DP dependency for batch clipping with shuffling.

==> Section/01_RelatedWork.tex <==
\section{Related Work}
\label{sec:01relatedwork}
{\color{red}TODO: add clipping methods in DPSGD papers}

{\color{red}TODO: add some privacy budget results from DPSGD papers}
% {\color{red}TODO: add different clipping methods in DPSGD papers}
{\color{red}TODO: add CIFAR10 comparisons table}


\begin{table}[H]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
 Method  & Model & Optimizer & $s$& $k$ &Test Accuracy & $(\epsilon,\delta)$ & BN layers\\ \hline
 DP-FTRL  & Convnet $(3C+2FC)$ & DP-FTRL & $2000$& $20$ & $70\%$ & $(20,1e-6 )$ & No\\ \hline
 Varun et al & Convnet $(2C + 2FC)$ & DPSGD & $64$ & $51$ & $ 51\%$ & $N/a$ &\\ \hline
 DPSGD(IC) & Convnet $(4C + 1FC)$  & DPSGD & $64$ & $50$ & $38.1\%$ & $( 0.5353, 1/50000)$ & No\\ \hline
 DPSGD(IC) & VGG16  & DPSGD & 2 & $50$ & 3& 4 & No\\ \hline
 DPSGD(BC) & Convnet $(4C + 1FC)$  & DPSGD & 2 & $50$ & 3& 4 & No\\ \hline
 DPSGD(BC + BN)  & Convnet & DPSGD & 2 & $50$ & 3& 4 & Yes\\ \hline
 DPSGD(BC)  & VGG16 & DPSGD & 2 & $50$& 3 & 4 & Yes\\ \hline
 DPSGD(BC + BN)  & VGG16 & DPSGD & 2 & $50$ & 3& 4 & Yes\\ \hline
\end{tabular}
\caption{Performance Comparison CIFAR10}
\label{table:Related_works}
\end{table}



==> Section/02_DPSGD_with_individual_clipping.tex <==
\section{DPSGD with Individual Clipping}
\label{subsec:02DPSGDwithIndividualClipping}

% \subsection{Differential Privacy w}
% \label{subsec:02differentialprivacy}
% {\color{red}TODO: Add Differential privacy definitions here}
Differential privacy \citep{dwork2006calibrating, dwork2011firm,dwork2014algorithmic,dwork2006our} defines privacy guarantees for algorithms on databases, in our case a client's sequence of mini-batch gradient computations on his/her training data set. The guarantee quantifies into what extent the output  of a client (the collection of updates communicated to the server) can be used to differentiate among two adjacent training data sets $d$ and $d'$ (i.e., where one set has one extra element compared to the other set).

\begin{defn} \label{defDP} A randomized mechanism ${\cal M}: D \rightarrow R$ is $(\epsilon, \delta)$-DP (Differentially Private) if for any adjacent $d$ and $d'$ in $D$ and for any subset $S\subseteq R$ of outputs,
$$ Pr[{\cal M}(d)\in S]\leq e^{\epsilon} Pr[{\cal M}(d')\in S] + \delta,$$
where the probabilities are taken over the coin flips of mechanism ${\cal M}$.
\end{defn}

The privacy loss incurred by observing $o$ is given by
$$ L^{o}_{{\cal M}(d) \| {\cal M}(d')} = \ln \left( \frac{Pr[{\cal M}(d)=o]}{Pr[{\cal M}(d')=o]} \right).
$$
As explained in \citep{dwork2014algorithmic} $(\epsilon, \delta)$-DP ensures that
for all adjacent $d$ and $d'$ the absolute value of privacy loss will be bounded by $\epsilon$ with probability at least $1-\delta$. 
The larger $\epsilon$ the more certain we are about which of $d$ or $d'$ caused observation $o$. 
When using differential privacy in machine learning we typically use $\delta=1/N$ (or $1/(10N)$) inversely proportional with the data set size $N$.

In order to prevent data leakage from  inference attacks in machine learning \citep{lyu2020threats} such as the deep leakage from gradients attack
\citep{ligengzhu201deepleakage,zhao2020idlg,geiping2020inverting} or the membership inference attack
\citep{shokri2017membership,nasr2019MIA,song2019MIA} a range of privacy-preserving methods have been proposed. 
Privacy-preserving solutions 
for federated learning are Local Differential Privacy (LDP) solutions \citep{abadi2016deep,abhishek2018privateFL,mohammad2020privateFL,stacey2018privateFL,meng2020privateFL,duchi2014local} and Central Differential Privacy (CDP) solutions \citep{mohammad2020privateFL,robin2017privateFL,mcmahan2017learning,nicolas2018privateFL,Yu2019CDP}. 
In LDP, the noise for achieving differential privacy is computed locally at each client and is added to the updates before sending to the server -- in this paper we also consider LDP. In CDP, a trusted server (aka trusted third party) aggregates received client updates into a global model; in order to achieve differential privacy the server adds noise to the global model before communicating it to the clients.  
\subsection{Deep Learning}
\label{subsec:02deeplearning}
{\color{red}TODO: Add Deep Learning models descriptions here}
\subsubsection{Image Classification}
\subsubsection{Shuffling Stocastic Gradient Descent}
\subsection{DPSGD}
{\color{red}TODO: Shows Abadi's individual clipping algorithm here}

==> Section/03_Differential_Privacy.tex <==
\section{Gaussian Differential Privacy}
\label{subsec:03GaussianDifferentialPrivacy}

==> Section/04_DPSGD_with_batch_clipping.tex <==
\section{DPSGD with Batch Clipping}
\label{sec:04DPSGDwithBatchClipping}


%%%% Shuffling Batch clipping algorithm %%%%%%
\begin{algorithm}[H]
\caption{Shuffling Batch Clipping DPSGD}
\label{alg:fed_batch_FL_DPs}
\begin{algorithmic}[1]
%\Procedure{LocalSGDwithDP}{$d,C,s,\sigma,T$}
\Procedure{Shuffling\_BatchClippingDPSGD}{}
    \State \textbf{Input:} dataset (D), batch size (s), number of epochs (K), learning rate ($\eta$), Gradient norm bound (C), noise scale $\sigma$, loss function L, model seed $\hat{w}_0$
    % \State N = len(D) \Comment{Get total number of rows in data set D}
    \State batches = divide\_dataset\_to\_batches(D,s) \Comment{detach dataset into equally data batches}
    \State B = len(batches)
    \For{batch \textbf{in} batches}
        \State normalize(batch) \Comment{Normalize data in each batch}
    \EndFor
    \For{k$= 0,1,2,\dots,K-1$}
        \State batches = shuffle(batches)
        \For{$b = 0,1,2,\dots, B-1$}
        \State $w=\hat{w}$
            \State U = 0
            \State batch = shuffle(batches[b])
            \For{$t = 0,1,\dots, s/m-1$}
                \State $g =\frac{1}{m} \sum_{i=0}^{m} \nabla L(w,batch[tm+i])$
                \State $w \leftarrow  w - \eta_{kB+b} \cdot g$
                \State $U \leftarrow U + g$
            \EndFor
            \State $U \leftarrow [U]_C$
            %$U/ \max(1,\frac{||U||_2}{C})$ 
            \Comment{Clipping gradient}
            \State $U\leftarrow U + N(0,C^2 \sigma^2 \textbf{I}) $ \Comment{Add noise to clipped gradients}
            \State $\hat{w} \leftarrow \hat{w} - \eta_{kB+b} \cdot U$
        \EndFor
    \EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}

[TO DO: explain leakage model of DPSGD and for us model $\hat{w}$ can be queried (not $w$)]

%%%% Shuffling individual clipping algorithm %%%%%%
\begin{algorithm}[H]
\caption{Shuffling Individual Clipping DPSGD}
\label{alg:fed_batch_FL_DPs}
\begin{algorithmic}[1]
%\Procedure{LocalSGDwithDP}{$d,C,s,\sigma,T$}
\Procedure{Shuffling\_IndividualClippingDPSGD}{}
    \State \textbf{Input:} dataset (D), batch size (s), number of epochs (K), learning rate ($\eta$), Gradient norm bound (C), noise scale $\sigma$, loss function L, model seed $\hat{w}_0$
    % \State N = len(D) \Comment{Get total number of rows in data set D}
    
%    \For{batch \textbf{in} batches}
%        \State normalize(batch) \Comment{Normalize data in each batch}
%    \EndFor
    \For{k$= 0,1,2,\dots,K-1$}
        \State D = shuffle(D)
        \State batches = divide\_dataset\_to\_batches(D,s) \Comment{detach dataset into equally data batches}
        \State B = len(batches)
 %       \State batches = shuffle(batches) ??? TO DO: shuffle over the whole data set, and then partition into batches, copy line 4 to here
        \For{$b = 0,1,2,\dots, B-1$}
        \State $w=\hat{w}$
            \State U = 0
            \State batch = batches[b] %shuffle(batches[b])
           \For{$t = 0,1,\dots, s-1$}
                \State $g =\nabla L(w,batch[t])$
                % \State $[g]_C = g/ \max(1)$
                \State $g\leftarrow [g]_C$
%                \State $w = w - \eta \cdot g$
                \State $U \leftarrow U + g$
            \EndFor
%            \State $U_c = U/ \max(1,\frac{||U||_2}{C})$ \Comment{Clipping gradient}
            \State $U \leftarrow U + N(0,C^2 \sigma^2 \textbf{I}) $ \Comment{Add noise to clipped gradients}
            \State $\hat{w} \leftarrow \hat{w} - \eta_{kB+b} \cdot U$
        \EndFor
    \EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}

[TO DO: explain how the original individial clipping is captures ($1/s$ into $\eta$)]

[TO DO: transfer of batch normalization from other publicized data set; or need DP version of batch normalization; or one does what we do]

[TO DO: what about the feature map based on PCA -- also this needs to be DP, or transferred]

[TO DO: ?? last theorem DPSGD paper -- what is meant by hyperparameters (topology of the model etc., or also PCA computations?)]
% \subsection{Masked Gradients}
% For the new masking algorithm, I am not that certain any more and somehow I cannot reproduce what I had in my mind. We should discuss. Right now I am thinking in the following confusing ways:

% We know from our Hogwild! analysis that we can partition the entries of a gradient vector in $D$ parts and select one of these at random -- and still yield 'optimal' convergence. For the selected part we keep the entries in the gradient. The non-selected parts are masked, that is, the entries in the gradient are set to zero.
 
% For strongly convex problems this leads to a factor $D$ slower convergence and this means we need $k'=kF$ epochs local gradient computations. The lower bound on $T$ is now a factor $D^2$ larger and this means a factor $D^2$ more rounds. This is fine if a solution for the sample size sequence exists: We recompute $\bar{s}'=\bar{s}/D$, hence, D can be at most $\bar{s}$.

% We used to clip the norm of the gradient down to $C$. But this is for all $D$ parts together. Each part can be seen to be separately clipped to $C' = C / \sqrt{D}$. And this is what will use for the masked gradient.

% Notice that $C'^2 (\sigma \sqrt{D}) ^2 = C^2 \sigma^2$. So, we keep the same noise as before. However, now the noise after renormalization with $C'$ yields a differential privacy noise of $\sigma*\sqrt{D}$. This gives a better (smaller) $\epsilon$. A huge improvement.

% We hope that the theory for strongly convex problems extrapolates to plain convex and non-convex problems.

% Rather than selecting one of $D$ parts at random, we can do better and only keep the part with the largest entries -- better convergence is expected. Or even better, we simply take the gradient and only keep the $D$ largest entries (in absolute values).

% There is one confusing aspect: We also know that the clipping constant cannot be arbitrarily reduced, hence, also $C'$ should be 'large enough'. By choosing a random part, we guarantee that our formula for $C'$ matches the effect of $C$ in the original distributed SGD algorithm, hence, if $C$ is large enough in the original setting, $C'$ will be large enough in this new masked setting. This argument shows that selecting a random part as strategy may be prefered.

% In the above analysis we push $D$ to $\bar{s}$ which makes $\bar{s}'=1$, that is, a single iteration. We also know that too small mini-batch or sample size does not work too well. Hence, we may only be able to use $D=\bar{s}/\text{large-enough-constant}$. A sensitivity study will help here.

% Notice that T meets our lower bound and this gives $\bar{s}=(N/k)/\text{const}$, that is, $\bar{s}'= (N/(Dk))/\text{const}$.

% The algorithm will work as follows:

% = We a-priori select a partition of vectors in $D$ parts.

% = We select one part at random and zero out the entries of the gradient in the other parts.

% = We clip the masked gradient by using clipping constant $C/\sqrt{D}$.

% = As before we add the masked-clipped gradients of the sample (mini-batch) together and add $N(0,C^2\sigma^2)$ noise. This will be the local round update $U$ with noise.


% \subsection{Diminishing Clipping constants}
% Main Goal: we want to have a decreasing sequence of clipping constants. We denote $M_i$ the decreasing sequence. $M_i$ has to be defined based on previous iterations, i.e., $0, 1,\dots, i-1$. We can use moving average to implement $M_i$.  

% Another really good idea in this line of thinking: Let $\bar{\eta}_i$ be the round step size.  We know we compute $s$ gradients in a single round. Suppose these gradients all have norm $n_i$. After aggregating the gradients, we see at most a norm $$\sqrt{s} \times n_i$$ and this is realized if all $s$ gradients sort of point into the ``same'' direction. We equate this to $$\bar{\eta}_i=\sqrt{s} \times n_i$$ and in this way we replace multiplying with the step-size by clipping with $n_i$. We still add the noise $$C\times \sigma \times \bar{\eta_i}$$ as before. This 
% implicitly includes multiplying with the step size $\bar{\eta}_i$. 
% We have $n_i=\bar{\eta}_i / \sqrt{s}$. The effective noise is now $$(C*\sigma*\bar\eta_i)/n_i = C*\sigma*\sqrt{s} = \sigma'.$$ This is very large. Notice that all of C is included and an extra $\sqrt{s}$ factor.

% Usually C is less than 1, say 0.1 or so. So, for this to work, we want $s>=100$.

% Now we always do clipping as this replaces multiplying with the step size. This also means we use the DP theory in a tight way (since this always pushes to the worst-case scenario for each data sample).

% Summarizing: We clip gradient with $$n_i=\bar\eta_i/\sqrt{s}$$ and we add noise $$\bar\sigma*\bar{\eta}_i$$ to the aggregated update at the end of the round. Here, $\bar{\sigma}$ plays the role of $C*\sigma$. And in our DP theory we use $$\sigma' = \bar{\sigma}*\sqrt{s}.$$


% % Toan comments

% DPSGD: $N(0, C^2 sigma^2 I)$
% this paper: $N(0, \bar{\sigma}^2)$

% $n_i = C'$: norm of 1 gradient.
% $new_sigma$ = $variance / n_1$
% $new_para = para + lr * (gradient + noise)$   

% 1. Standard format: $N(0,(C\sigma)^2)$ where $C\sigma$ is the variance of the noise and $C$ is the max norm of one gradient.  

% 2. At the $i$-th iteration, we have maximum norm of one gradient is $n_i$ or $C_i = n_i$. In this case, the aggregated norms is equal to $\sqrt{s}*n_i$ because we have $s$ gradients. The reason is very simple when we update the parameters, the information of $s$ gradients. Actually, $C_i = min(C,n_i)$.

% 3. Then I define $\bar{\eta}_i = \sqrt{s}*n_i$ and we can be sure that $n_i$ will get smaller by time. 

% We define stepsize $\bar{\eta}_i$ and from there, we can know $n_i$ or we can do reversely, compute $n_i$ and then we calculate $\bar{\eta}_i$

% 4. We say we want to create a new noise with variance $C\sigma \bar{\eta}_i$, then what is $C$ and $\sigma$ in this case? We may want to define $C = n_i$ because $n_i$ is the max norm of one gradient at the $i$-th iteration. From here, we already now noise variance:= $$C\sigma=n_i \sigma=C\sigma \bar{\eta}_i$$

% It means $\sigma$ or $\sigma' = C \sigma \sqrt{s}$. 

==> Section/05_BatchClipping_DP_Analysis.tex <==
\section{Batch Clipping DP Analysis}
\label{sec:05DPSGDbatchclippingDPanalysis}
{\color{red}TODO: This section shows how we build an accountant to compute the privacy budget $(\epsilon,\delta)$}

==> Section/06_Hyperparameters_configuration.tex <==
\section{Hyperparameters Configuration}
\label{sec:06hyperparametersconfiguration}

{\color{red}TODO: This section shows how we choose the hyperparameters in the experiments}

==> Section_old/00_Introduction.tex <==

%\section{Proofs place holder}

\section{Introduction}

%Privacy leakage is a big problem in the big-data era.
%Solving a learning task based on big data intrinsically means that only through a collaborative effort sufficient data is available for training a global model with sufficient clean accuracy (utility).
%Federated learning is a framework where a learning task is solved by a loose federation of participating devices/clients which are coordinated by a central server \citep{mcmahan,jianmin,bonawitz2019towards,konevcny2016federated,GoogleAIBlog,yang,luping,kevin,cong2019,yang2019,tianli2019hetero,lian2015asynchronous,lian2017asynchronous,ManiaPanPapailiopoulosEtAl2015,DeSaZhangOlukotunEtAl2015,jie2020asynchronous}.
%Clients, who use own local data to participate  in a learning task by training a global model, want to have privacy guarantees for their local proprietary data. For this reason DP-SGD \citep{abadi2016deep} was introduced as it adapts distributed Stochastic Gradient Descent (SGD)\citep{nguyen2018sgd,nguyen2018new} with Differential Privacy (DP)\citep{dwork2006calibrating, dwork2011firm,dwork2014algorithmic,dwork2006our}.

In order to defend against privacy leakage of local proprietary data during collaborative training of a global model as in federated learning \citep{mcmahan},
%,jianmin,bonawitz2019towards,konevcny2016federated,GoogleAIBlog,yang,luping,kevin,cong2019,yang2019,tianli2019hetero,lian2015asynchronous,lian2017asynchronous,ManiaPanPapailiopoulosEtAl2015,DeSaZhangOlukotunEtAl2015,jie2020asynchronous}, 
\citep{abadi2016deep} introduced  DP-SGD  as it adapts distributed  Stochastic Gradient Descent (SGD)\citep{nguyen2018sgd,nguyen2018new} with Differential Privacy (DP)\citep{dwork2006calibrating, dwork2011firm,dwork2014algorithmic,dwork2006our}.

This approach allows each client to perform local SGD computations for the data samples $\xi$ that belong to the client's local training data set $d$. %The updates as a result of the SGD computations are sent to a centralized server who aggregates all received updates and maintains a global model. The server regularly broadcasts its most recent global model so that clients can use it in their local SGD computations. 
%This allows each client to use what has been learned from the local data sets at the other clients. This leads to good accuracy of the final global model.
%
Each client is doing SGD computations for a batch of local data. These recursions together represent a local round and at the end of the local round a local model update (in  the form of an aggregate of computed gradients during the round) is transmitted to the server. The server in turn adds the received local update to its global model -- and once the server receives new updates from (a significant portion of) all  clients, the global model is broadcast to each of the clients. When considering privacy, we are concerned about how much information these  local updates reveal about the used local data sets. 
%Each client wants to keep its local data set as private as possible with respect to the outside world which observes round communication (the outside world includes all other clients as well).

Depicted in Algorithm \ref{alg:genDPSGD} (a detailed description and explanation is given in Section \ref{sec:alg}), we introduce a general algorithmic framework of which DP-SGD is one example. The main generalization beyond DP-SGD is that the most inner loop can execute any optimization algorithm ${\cal A}$ in order to compute a local round update $U$. 
%The algorithmic framework for 
%VVV
DP-SGD is realized for $s=1$ with ${\cal A}$ computing a single gradient:
%Before adding Gaussian noise, this yields the local update
\begin{equation}
    U = \sum_{i\in S_b} [ \nabla f(w,\xi_{i})]_C, \label{indclip}
\end{equation}
where $[x]_C= x/\max\{1,\|x\|/C\}$ is the clipping operation and $S_b$ is a batch sampled from  local data set $d$ of size $m$.
%(in the notation of the algorithmic framework, $S_b=\bigcup_{h=1}^m S_{b,h}$ where $|S_{b,h}|=s=1$ represent single data samples). 

We call (\ref{indclip}) the {\em individual clipping} approach and  notice that it implements mini-batch SGD. This is necessary because the DP analysis requires each clipped output to be independent from other clipped outputs. This implies that computation of one clipped output should not involve updating a local model $w$ which is used in a computation of another next clipped output. This means that each of the clipped gradients in the sum are evaluated in the same $w$ (the most recently received global model from the server). 
%The main disadvantage of mini-batch SGD is that it does not converge as fast as other SGD-based algorithms such as classical SGD. It is not the individual clipping (with a fine-tuned clipping constant $C$) but mainly the mini-batch SGD approach that makes convergence slow. 
We notice that the clipping operation introduces `clipping' noise and together with the added Gaussian noise for differential privacy this results in convergence to a final global model with smaller (test) accuracy (than what otherwise, without DP, can be achieved).

Our algorithmic framework allows a much wider choice. In particular,  $m=1$ 
%VVV and $v=1$ yields
allows for example
\begin{equation}
U = [\sum_{j=1}^s \nabla f(w_j,\xi_{i_j})]_C, \label{batchclip}
\end{equation}
where $S_b=\{i_1,\ldots, i_s\}$ is a batch sampled from the local data set $d$ of size $s$ and where algorithm ${\cal A}$ implements classical SGD according to the SGD recursion
$$ w_{j+1}=w_j-\eta \nabla f(w_j,\xi_{i_j}),$$
where $w_1=w$ is initialized by the most recently received global model from the server (possibly updated with updates send to the central server, see lines 8 and 24 in Algorithm \ref{alg:genDPSGD}) and where $\eta=\eta_{(e-1)\frac{N}{ms}+b}$ is the round step size (for round $b$ in epoch $e$). 

We call (\ref{batchclip})  an example of {\em batch clipping}. Batch clipping in its most general form is
\begin{equation}
    U= [{\cal A}(w,\{\xi_i\}_{i\in S_{b}})]_C.
    \label{batchclipA}
\end{equation}
It allows us to implement classical SGD
%~\citep{nguyen2018sgd,nguyen2021unified} 
and go beyond mini-batch SGD such as Adam~\cite{kingma2014adam}, AdaGrad~\cite{duchi2011adaptive}, SGD-Momentum \cite{sutskever2013importance}, RMSProp \cite{zou2018sufficient}. The framework is general in that ${\cal A}$ can implement any optimization algorithm including classical (as discussed above) or momentum based SGD type algorithms.



%==========================
%
%\textcolor{red}{See paragraph above, is the explanation correct?}
%
%\textcolor{red}{Ha to Marten} 
%
%= Short answer: your writing is correct. 
%
%= Long answer: Here is the information from Toan. DP-SGD is implemented in the software package called Opacus and written by Facebook. This package is built on the top of another software package called pytorch. This pytorch is optimized for normal mini-batch like optimizers such as SGD, etc. But not for individual clipping one/ Opacus. Therefore, the implementation of Opacus is not optimal at all. Precisely, for normal mini-batch SGD with batch size $m$, we may need $O(n)$ memory complexity where $n$ is the size of network and it is very big in practice. In Opacus, the memory is $O(mn)$ and thus, memory becomes a critical thing. 
%
%@Toan: what is your input?
%
%===============================


%%%% Shuffling Batch clipping algorithm %%%%%%
\begin{algorithm}[t]
\caption{%Differential Private SGD -- 
Generalized Framework for DP-SGD}
\label{alg:genDPSGD}
\begin{algorithmic}[1]
%\Procedure{LocalSGDwithDP}{$d,C,s,\sigma,T$}
\Procedure{DP-SGD-General}{}
%    \State \textbf{Input:} dataset (D), batch size (s), number of epochs (K), learning rate ($\eta$), Gradient norm bound (C), noise scale $\sigma$, loss function L, model seed $\hat{w}_0$
    % \State N = len(D) \Comment{Get total number of rows in data set D}
    \State $N=$ size training data set $d=\{\xi_i\}_{i=1}^{N}$
    \State $E=$ total number of epochs
 %   \State $\{C_e\}_{e=1}^{E1}$ sequence of clipping constants (per epoch)
    \State $T=$ total number of rounds
    \State diminishing round step size sequence $\{\eta_i\}_{i=1}^{T}$
    \State 
    \State initialize $w$ as the default initial model
    \State {\bf Interrupt Service Routine (ISR)}:  Whenever a new global model $\hat{w}$ is received, computation is interrupted and an ISR is called that replaces $w\leftarrow \hat{w}$ after which computation is resumed
    \State
    \For{$e\in \{1,\ldots, E\}$}
    \State Let $\pi^e$ be a random permutation 
    \State re-index data samples: $\{\xi_i\leftarrow \xi_{\pi^e(i)}\}_{i=1}^N$  
    \State $\{S_{b,h}\}_{b=1,h=1}^{N/(ms),m}\leftarrow$ ${\tt Sample}_{s,m}$ with \State \hspace{0.35cm} $S_{b,h}\subseteq \{1,\ldots, N\}$, 
    \State \hspace{0.35cm} $|S_{b,h}|=s$, $|S_b|=sm$ with $S_b=\bigcup_{h=1}^m S_{b,h}$ 
    \For{$b\in \{1,\ldots, \frac{N}{ms}\}$}
%    \State Set $w$ equal to last received global model
 %   \State $U=0$
 \State Start of round $(e-1)\frac{N}{ms}+b$:
    \For{$h\in \{1,\ldots m\}$}
    \State $a_h\leftarrow {\cal A}(w,\{\xi_i\}_{i\in S_{b,h}})$
 %   \State $U\leftarrow U+[a]_C$
    \EndFor
    \State $U=\sum_{h=1}^m [a_h]_C$
    \State $\bar{U}\leftarrow U+ {\cal N}(0,(2C\sigma)^2{\bf I})$
    \State Transmit $\bar{U}/m$ to central server
    \State Locally update $w\leftarrow w- \eta_{(e-1)\frac{N}{ms}+b} \cdot \bar{U}/m$
    \EndFor
    \EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}

We have two main contributions: 
%
%We introduce a general algorithmic framework and introduce a new proof technique 
%for a slightly stronger adversary compared to DP proofs in current literature 
%that allows us to characterize tight $f$-DP guarantees in simple formulas: 
%and we introduce a new differential privacy amplification method based on computing the moving average of round updates before transmitting to the server.

\noindent
{\bf General Algorithmic Framework:} Algorithm \ref{alg:genDPSGD} with detailed discussion  in Section \ref{sec:alg} defines our general framework. In the inner loop it allows execution of any optimization algorithm ${\cal A}$ of our choice. This covers classical SGD and momentum based SGD, and can possibly be extended with batch normalization (over $S_b$). Our framework is compatible with asynchronous communication between clients and server. We also notice that the framework allows diminishing step sizes (learning rate), and allows adapting the clipping constant from round to round (this is compatible with DP analysis in general).
    
%\item 
\noindent {\bf DP Proof Technique based on a Sampling Induced Distribution:} 
%Section \ref{sec:GDP} explains  $f$-DP \cite{dong2021gaussian} which we use to analyze our general algorithmic framework. 
We introduce a {\em slightly} stronger adversary, denoted by ${\cal A}_1$ in Table \ref{tab:DP}, compared to the model, denoted by ${\cal A}_0$ in Table \ref{tab:DP}, used in DP proofs in current literature. The adversary knows how ${\sf Sample}_m$ operates and can derive a joint probability distribution $\mathbb{P}$ of the number of differentiating data samples for each round within the sequence of rounds that define the series of epochs during which updates are computed. DP analysis based on ${\cal A}_0$ considers each round separately and analysis of a single round assumes a strong adversary who knows the instance drawn from the projection of $\mathbb{P}$ on that round (analysis of the whole sequence of rounds follows from composition of the derived DP guarantees of single rounds). Our DP analysis based on ${\cal A}_1$ deals with the whole sequence of rounds at once and the resulting analysis assumes a slightly stronger adversary who knows the instance drawn from $\mathbb{P}$. Appendix \ref{sec:adv} discusses the adversarial models in more detail.
%and shows an asymptotic comparison indicating into what extent "W" can lead to a better DP guarantee
    
We introduce a probability distribution $q_E(c)$ induced by the sampling procedure ${\sf Sample}_{s,m}$. Together with the knowledge of an instance of $\mathbb{P}$ given to our slight stronger adversary in our DP analysis, 
%DP analysis the stronger adversary  is given knowledge of the instance drawn from $q_E(c)$ (  
we prove an $f$-DP guarantee \citep{dong2021gaussian} where $f$ is related to a mix of Gaussian trade-off functions $G_{c/\sigma}$ according to distribution $q_E(c)$. 
    
Table \ref{tab:DP} summarizes our results which we interpret in  Section \ref{sec:DPanalysis}.
Our DP analysis shows that a much wider class of SGD based algorithms have provable DP guarantees. We remove the constraints made in the original DP-SGD paper; we can go beyond mini-batch SGD and we may replace random subsampling by shuffling. We see that in $f$-DP terminology various configurations in the general algorithmic framework provide a $\approx G_{\sqrt{gE}/\sigma}$-DP guarantee with a $\sqrt{gE}$ dependency, where we consider group privacy for groups of size $g$, $E$ is the total number of epochs (measured in data set size $N$) worth of gradient computations, and $\sigma$ characterizes  the added Gaussian DP noise (after normalization with the clipping constant). This square root dependency, in particular for group privacy (here shown for the first time),
%for groups of size $g$, 
must as a consequence also hold for the weaker ${\cal A}_0$ adversary.
%We show that the DP guarantee is invariant with respect to the number of rounds per epoch. 






%\item {\bf DP Amplification based on a Moving Average over Round Updates:} Let $U_b$ be the update computed in round $b$ before adding Gaussian noise. Rather than adding Gaussian noise to $U_b$ and transmitting the result to the server, we propose computing the moving average 
%$$ \frac{1}{a}\sum_{j=0}^{a-1} U_{b-j},
%$$
%add Gaussian noise, and next transmit the result to the server. We show that this approach is into some extent the same as multiplying parameter $m$ in Algorithm \ref{alg:genDPSGD} by $a$, except for one crucial difference: The moving average uses/computes round updates $U_{b-j}$ where $U_{b-j}$ use the local model $w$ at the start of round $b-j$. These local models are updated from one to the next and this allows a more directed search towards the global minimum. Simply multiplying parameter $m$ by $a$ loses this benefit (here, all computations need to use the same local model). 



%The moving average enjoys the amplification effect of subsampling:
%Table \ref{tab:DP} shows how the $f$-DP guarantee improves with a factor $\sqrt{a}$, details are given in Section \ref{sec:MA}. Besides obtaining a better DP guarantee, one can use a larger $a$ to compensate for choosing a larger clipping constant $C$ and choosing a smaller $\sigma$ such that the standard deviation $2C\sigma$ of the Gaussian noise decreases. This reduces the clipping noise and Gaussian noise per round and is expected to yield convergence to a final global model with higher (test) accuracy. The disadvantage of using a larger $a$ is a delay in information transmission of the updates to the server which, if $a$ is not too large, is expected to have a minimal effect on the accuracy of the final global model \cite{nguyen2018sgd}.

%We notice that each client can easily (adaptively) adjust the moving average parameter $a$ for better fine tuning.
%\end{enumerate}


%TO DO split in the three main types of contributions (see abstract)

%Our main contribution is applying  $f$-DP to our general algorithmic framework which allows clipping a sum of computed outputs based on a batch of data samples:
%%[TO DO: update, make also sure group privacy and individual privacy is clear]
%\begin{itemize}
%    \item We introduce a new proof technique that uses a probability distribution induced by the used sampling strategy. Our DP analysis holds for any algorithm ${\cal A}$ including classical SGD and momentum based SGD, and possibly extended with batch normalization (over $S_b$). Our framework is compatible with asynchronous communication between clients and server.  
%    \item We analyze general sample strategies. DP-SGD uses subsampling. Another sampling strategy is shuffling which gives shuffling SGD. We show that both strategies (for either individual clipping or batch clipping) lead to approximately the same DP guarantees when neighboring data sets are considered. 
%    \item The resulting DP guarantees have simple closed form formulas that are easily evaluated (contrary to existing $f$-DP guarantees which are based on the more complex subsampling operator and composition tensor).
%    \item Our theory can be applied to analyzing group privacy leading to simple evaluable bounds for batch clipping.
%    %a non-closed formula for the DP guarantee). 
%    We show that group privacy for batch clipping scales with the square root of the size  of the group, while group privacy for individual clipping has a worse dependence. 
%    %We still have DP guarantees that scale with the square root of the total number of epochs.
%    
%    \item We show that  DP guarantees (for both neighboring data sets and group privacy) scale with the square root of the total number of epochs, and is not dependent on the explicit number of rounds executed within these epochs. In other words, even though more local updates can be observed by the adversary, this turns out not to lead to more privacy leakage. This is because each local update is based on a smaller batch of training data samples which in itself leads to less privacy leakage per local update.
%    %scales linearly in the group size.
%%    \item We analyze the effect of data normalization on the DP guarantee.
%
%\item Precise results are listed in Table \ref{tab:DP} and discussed in Section \ref{sec:DPanalysis} where the above contributions are shown to be implied by the results in the table.
%
%\item filtering technique ...
%
%\item remark factor 2 somewhere
%\end{itemize}

%TO DO EXPLAIN TABLE: Refer to section 3 and 3.1 for $f$-DP and the Gaussian trade-off function, also need to explain group privacy. Put translation into eps delta DP in intro? ; we also introduce a new bounding technique ; table also talks about general clipping 


\begin{table*}[t]
    \centering
{\small 
    \begin{tabular}{|ccc|cc|c|c|c|}
    \hline 
    \parbox[t]{2mm}{\rotatebox[origin=c]{90}{\hspace{1mm} ind. clipping (\ref{indclip}) \hspace{1mm}}} &
    \parbox[t]{2mm}{\rotatebox[origin=c]{90}{\hspace{1mm} batch clipping (\ref{batchclip}), (\ref{batchclipA}) \hspace{1mm}}} &
    \parbox[t]{2mm}{\rotatebox[origin=c]{90}{\hspace{1mm} gen. clipping (\ref{eq:genA}), (\ref{eq:gen}) 
    \hspace{1mm}}} &
    \parbox[t]{2mm}{\rotatebox[origin=c]{90}{\hspace{1mm} subsampling \hspace{1mm}}} &
    \parbox[t]{2mm}{\rotatebox[origin=c]{90}{\hspace{1mm} shuffling \hspace{1mm}}} &
    \parbox[t]{2mm}{\rotatebox[origin=c]{90}{\hspace{1mm} group privacy \hspace{1mm}}} &
    $h$-DP guarantee 
     & 
    \parbox[t]{2mm}{\rotatebox[origin=c]{90}{\hspace{1mm} adversarial model \hspace{1mm}}}  \\
    \hline
    \hline
         \vspace{-3mm} &  &  &  &  &  & &  \\
    x & & & x & & $g=1$ & $h=C_{m/N}(G_{1/\sigma})^{\otimes (N/m)\cdot E}$ from \cite{dong2021gaussian},
    %\approx G_{\sqrt{E}/\sigma}$, approximation is  
    & ${\cal A}_0$ \\
    &&&&&& the {\em original DP-SGD setting} \cite{abadi2016deep} & \\
    \hline
    \hline
        \vspace{-3mm} &  &  &  &  &  & &  \\
    x & & & x & & $g\geq 1$ & $h$ is in the range  $\approx \left[G_{\sqrt{(e+\gamma) \min\{m,g\} g E}/\sigma}, (\alpha \rightarrow 1-\alpha)\right]$, & ${\cal A}_1$ \\
    &&&&&& approximation is for small $e^{-\gamma g E}$  & \\
        \vspace{-2mm} &  &  &  &  &  & &  \\
     & x & & x & & $g\geq 1$ & $h$ is in the range $\approx \left[G_{\sqrt{(1+1/\sqrt{2gE})gE}/\sigma}, G_{\sqrt{(1-1/\sqrt{2gE})gE}/\sigma}\right]$, & ${\cal A}_1$ \\
     &&&&&& approximation is for small $e^{-gE}$ and small $s/N$ & \\
     &&&&&& (see Thm \ref{thm:shuffling} for a tighter lower bound corresponding to Def \ref{def:f}) &\\
         \vspace{-2mm} &  &  &  &  &  & &  \\
     & & x & x & & $g=1$ & $h$ is in the range $\approx \left[G_{\sqrt{(1+1/\sqrt{2E})E}/\sigma}, G_{\sqrt{(1-1/\sqrt{2E})E}/\sigma}\right]$, & ${\cal A}_1$\\
     &&&&&& approximation is for small $e^{-E}$ & \\
         \vspace{-2mm} &  &  &  &  &  & &  \\
     & & x & & x & $g=1$ & $h=G_{\sqrt{E}/\sigma}$ & ${\cal A}_1$ \\
         \vspace{-2mm} &  &  &  &  &  & &  \\
     & & x & & x & $g\geq 1$ & $h$ is in the range $\approx [G_{\sqrt{gE}/\sigma}, (\alpha \rightarrow 1-\alpha)]$, & ${\cal A}_1$\\    &&&&&&    
         approximation is for constant $E$ and  small $g^2ms/(N-g)$ &\\
  \vspace{-2mm} &  &  &  &  &  &   & \\        
     & x &  & & x & $g\geq 1$ & $h \in \left[G_{\sqrt{gE}/\sigma}, (\alpha \rightarrow 1-\alpha)\right]$ & ${\cal A}_1$ \\
         \vspace{-2mm} &  &  &  &  &  & &  \\
     & x &  & & x & $g\leq s$ & $h \approx G_{\sqrt{gE}/\sigma}$, & ${\cal A}_1$ \\
     &&&&&& approximation is for constant $E$ and
     %$g\leq s$ and 
     small $g^2/(N/s-g-g^2)$ & \\
 %        \vspace{-3mm} &  &  &  &  &  &   \\
    \hline
%    \hline
%            \vspace{-2mm} &  &  &  &  &  &   \\
%    &&&&&& {\em With moving average for parameter $a$:}
%         \vspace{-2mm} &  &  &  &  &  &   \\
%     & & x & & x & $g=1$ & $h=G_{\sqrt{E}/(\sqrt{a}\cdot \sigma)}$ \\
%         \vspace{-2mm} &  &  &  &  &  &   \\
%     & & x & & x & $g\geq 1$ & $h$ is in the range $\approx [G_{\sqrt{gE}/(\sqrt{a}\cdot \sigma)}, (\alpha \rightarrow 1-\alpha)]$, \\    &&&&&&    
%         approximation is for constant $E$ and  small $g^2ams/(N-g)$ \\    
%    \hline
    \end{tabular}
}
    \caption{
    Trade-off functions $h$ for the mechanism ${\cal M}$ defined by Algorithm \ref{alg:genDPSGD} in the strong (${\cal A}_0$) or slightly stronger (${\cal A}_1$) adversarial model for all pairs of data sets $d$ and $d'$ 
with $\max \{ |d\setminus d'|, |d'\setminus d|\}\leq g$; 
%and $N=|d\cap d'|+g$; 
$h$ cannot be improved beyond the reported ranges closer towards function $\alpha \rightarrow 1-\alpha$ (which represents random guessing of the hypothesis $d$ or $d'$, hence, no privacy leakage). An approximation for a small quantity means that if the quantity tends to $0$, then the approximation becomes tight.}
    \label{tab:DP}
\end{table*}


\noindent
{\bf Outline:} Section \ref{sec:alg} defines our general algorithmic framework. The minimal necessary background on $f$-DP is in Section \ref{sec:GDPmain} (with a full description in \ref{sec:GDP}).
Section \ref{sec:DPanalysis} states the main definitions and main theorems (proved in Appendices \ref{sec:lemmas} and \ref{sec:DPproof} with a discussion on the used adversarial model in Appendix \ref{sec:adv}) together with a detailed discussion of the application of the main theorems in Table \ref{tab:DP} (with corresponding proofs/applications for the tabled cases in Appendices \ref{sec:subsampling} and \ref{sec:shuffling}). Section \ref{sec:07experiments} shows simulations for mini-batch SGD with individual clipping, batch clipping, and a mixed clipping that merges both approaches.  
The accuracy of each are comparable. The advantage of using batch clipping over individual and mixed clipping 
%which is allowed in our generalized framework 
is improved memory utilization. 
%demonstrates improved utility (accuracy). 
This shows that the full extent/flexibility of our framework is worth studying in future work.



%Our DP analysis shows that a much wider class of SGD based algorithms have provable DP guarantees. We remove the constraints made in the original DP-SGD paper; we can go beyond mini-batch SGD and we may replace random subsampling by shuffling. We show that the DP guarantee is invariant with respect to the number of rounds per epoch. 
%We also introduce the moving average technique when shuffling is used. 
%This allows (in theory) a significant boost in differential privacy while at the same time reducing clipping and Gaussian noise. 
%We also justify the use of data normalization.
%All this gives the engineer a wider choice for achieving practical accuracy.

%%%%%% NO %%%%%%%%%%%%%
%Table \ref{tab:DP} shows that we can achieve $\approx G_{\sqrt{gE}/\sigma}$-DP for group privacy of $g$ samples and a total of $E$ epochs total gradient computation. This does not reflect the role of the batch size $|S_b|=|\bigcup_{h=1}^m S_{b,h}|=sm$. This is implicitly captured in $\sigma$. 
%The following thought experiment shows how: Suppose we increase $m$ to $am$, a factor $a$ larger. Then the norm of updates $U$ will become a factor $a$ larger. As a result, with respect to convergence to and accuracy of the final global model, we should be able to cope with a factor $a$ larger Gaussian noise. That is, by keeping the relative amount of noise with respect to the norm of $U$ constant, the new updates corresponding to batch size $am$ can be noised with $a\cdot {\cal N}(0,(2C\sigma)^2{\bf I})={\cal N}(0, (2C a\cdot \sigma)^2{\bf I})$. This shows that we can use the factor $a$ for increasing (1) the clipping constant $C$ (which reduces the clipping noise which is prevalent at the start of DP-SGD so that convergence can more easily start) and/or increasing (2) the standard deviation $\sigma$ (which improves the $G_{\sqrt{gE}/\sigma}$-DP guarantee as it gets closer to $G_0$ for larger $\sigma$). 
%%%%%%%%%%%%%%%%%%%%%%%

%In other words, we can increase the clipping constant $C$ (which reduces the clipping noise so that convergence can more easily start) and/or the standard deviation $2C\sigma$ of the Gaussian noise per round update (which directly influences the accuracy of the final global model).

%Table \ref{tab:DP} shows that shuffling with a moving average over $a$ round updates achieves $\approx G_{\sqrt{gE}/(\sqrt{a}\cdot \sigma)}$-DP for group privacy of $g$ samples and a total of $E$ epochs total gradient computation.
%TO DO for MA: From the presented DP analysis we see that batch clipping with subsampling or shuffling leads to $\approx G_{\sqrt{gE}/\sigma}$-DP. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Without modifying $C$ or $\sigma$, the $a$ larger standard deviation yields $\approx G_{\sqrt{gE}/(a\cdot \sigma)}$-DP.
%According to \cite{dong2021gaussian}, see (\ref{eq:gdp}), this translates to 
%$(\epsilon, \delta(\epsilon))$-DP for all $\epsilon\geq 0$, where
%$$ \delta(\epsilon) = \Phi(-\frac{\epsilon a\cdot \sigma}{\sqrt{gE}}+\frac{\sqrt{gE}}{2 a\cdot\sigma}) - e^{\epsilon} \Phi(-\frac{\epsilon a\cdot\sigma}{\sqrt{gE}}-\frac{\sqrt{gE}}{2 a\cdot\sigma}).
%$$
%In this formulation we generally aim at $\delta(\epsilon)=1/N$ or $1/(10N)$. 
%We want to choose the clipping constant $C$ large enough in order to sufficiently reduce clipping noise, choose  $\sigma$ small enough so that $2C\sigma$ is small enough in that the `Gaussian noise per batch of $m$ samples in a round update' is sufficiently small, choose $a\geq \sqrt{gE}/\sigma$ large enough such that  solving  $\epsilon$ shows $\epsilon\leq 0.5$ or preferably an even smaller $\epsilon\leq 0.05$. DP-SGD  generally requires $\sigma$ to be relatively large, say $\sigma=10$, and this hurts proper convergence to an acceptable accuracy. 
%Our general algorithmic framework allows us to experiment with various SGD/optimization approaches in order to have faster convergence to a possibly higher accuracy -- this is left for future work.
%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Outline}

%Section \ref{sec:alg} explains the general algorithmic framework. Section \ref{sec:GDP} explains $f$-DP. Section \ref{sec:DPanalysis} summarizes our main theorems and results. 
%%Section \ref{sec:MA} explains the moving average technique.

%\textcolor{red}{very brief trade-off functions and Gaussian trade-off function; for the other operator and tensor refer to appendix; explain in relation to framework the adversarial model with asymptotic comparison; main definitions and theorems; table plus explanation; remove summary of table from intro -- explain that we can get {\em simple} closed form tight approximations for {\em new} algorithms as a result of the slightly stronger adversary and also show $\sqrt{g}$ dependency -- this gives lower bound for the weaker adversary considered in current f-DP, open problem how we can improve the bounds for the weaker adversary }

%The next sections explain the general algorithmic framework, provide the necessary $f$-DP background, prove DP guarantees for our framework, ..

%=========================


%\textcolor{red}{Ha to Marten and Toan} I have several important notes which I think they are missing in the paper and experiments. 

% DONE Let me talk about the original DP-SGD first. The original DP-SGD is presented in the moment account DP paper where people prove the privacy using Gaussian DP and moment account technique. To make the proof in the paper go through, all data point must be independent and thus mini-batch SGD is in need. Individual clipping only helps us to bound the sensitivity otherwise we cannot determine magnitude of Gaussian noise. One BIG negative point to DP-SGD is mini-batch SGD does not converge as fast as other SGD-based algorithm such as classical SGD, etc. What I want to say here is that individual clipping does not make the convergence of current DP-SGD converge slow. From the setting, the user has very limited choices when working with original DP-SGD. 


% Discussed in emails. \textcolor{red}{Toan:} the thing you want to compare is that you want to compare the current DP-SDG which does not have data normalization, runs mini-batch SGD with individual clipping to new setting where we can use data normalization, runs any type of training algorithm with individual/ batch clipping. We should see a clear win for new settings. 

% DONE Actually, what we try to show in this paper is NOT try to solve individual clipping vs batch clipping. What we want to show in this paper is that with new setting, we can provide a solid DP proof, we can use many different SGD-based algorithms, we can use individual/batch clippings. We remove all constraints made in the original DP-SGD paper.



% DONE The important question comes to us is that if we want to make the training faster, we have to abandon mini-batch SGD. It means we have to abandon the proof framework in DP-SGD paper. What is the framework? This is exactly what we are doing in this paper, we say let use Gaussian noise, $f$-DP notation and individual clipping or batch clipping, and any possible first other algorithm we can come up. @Marten: correct me if I am wrong, the main key in new proof framework is batch clipping trick. 



% DONE \textcolor{red}{Ha to Marten: we may want to present Algorithm 1 at very beginning and move all the text above below it because the text is basically used to describe Algorithm 1}

%============================







%motivation/related work; DP-SGD individual clipping, simplify pseudo code with math formulas, directly as sum of clipped gradients with added Gaussian noise, use ${\tt Sample}_s$ notation etc.; later pseudo code  for our batch clipping, with shuffling approach, and additional tweak is discussed in a later section.

%contributions: batch clipping, allows optimizations (original SGD iterations or whatever you want, no subsampling but shuffling SGD apporach, batch normalization layers can be analyzed, data normalization separate theory) and still have DP analysis, similar DP for $g=1$ (compare two formulas?), better DP for $g>1$, we simply and tight closed formula for $g=1$ and simple to compute formula for $g>1$. Did experiments ...

%Also address asynchronous framework, compatible.

%Outline:

%0) In intro: general algorithm with varying step sizes and epoch to epoch varying clipping constant, explain individual and batch clipping, explain sampling for subsampling (may create multisets) and shuffling

%explain sensitivity, explain why we can use any algorithm for the batch clipping and include batch normalization or other types of normalization wrt the batch if we want to. Also explain that the asynchronous framework applies.

%We provide a larger class of algorithms for which we can show DP !!

%1) Gaussian DP

%2) Additional lemmas: add lemmas on Gaussians

%3) [In the proofs below, create two trade-off functions for the two cases -- batch is part of the intersection or not at all, just use a Gaussian for both with different parameters, for now one of them uses $\mu=0$ and equals identity] subsampling for general g<=s (if larger g, then binomial argument less clean -- but can be done (will not do this here, because we want to show that shuffling SGD competes well and should be used in practice) ... g=1 over multiple epoch with sampling batches that are sets can be bounded, larger g, we may multiply and get more complex statement ... but now we see indeed multiplication with $g$ and batch clipping is doing better): apply lemmas to get upper and lower bounds and this relates to the framework's original formulas; explain how circ operator is worse; shuffling for g=1 with its immediate consequence; shuffling for general g apply lemmas; simpler bound using circ operator or assume worst-case with all differentiating samples in different batches, hence, we multiply with $\sqrt{g}$ which is much better than circ; compare both approaches -- shuffling is approximately the same as subsampling wrt DP leakage;

%4) data normalization: changes the trade-off function for one of the cases to a Gaussian based on sensitivity; provide bounds (the first one does not work well, but for $H_W$ and $H_D$ small we are okay -- hence, start with individual and later batch clipping); explain tweak

\section{Algorithmic Framework for Differential Private SGD} \label{sec:alg}

%TO DO: diminishing step sizes, adaptive clipping, post processing of $U$ before adding noise; remark adaptive clipping (DP median etc.; or using moving average); factor 2


We provide a general algorithmic framework for differential private SGD in Algorithm \ref{alg:genDPSGD}: 

%\vspace{2mm}

\noindent 
{\bf Asynchronous SGD:} We allow asynchronous communication between clients and the central aggregating server. Each client maintains its own local model. Each client implements an Interrupt Service Routine (ISR) which replaces its local model $w$ with any newly received
%\footnote{When the central server broadcasts a message containing $\hat{w}$ it should include a message number such that client ISRs can check whether a newly received $\hat{w}$ is indeed more recent than previously received global models.} 
global model $\hat{w}$ from the server. In practice asynchronous communication may lead to out of order arrival or dropped global models broadcast by the central server. A limited amount of asynchronous behavior 
%still 
leads to provably optimal convergence rates for certain learning tasks \cite{van2020hogwild}.

%\vspace{2mm}

\noindent 
{\bf Sampling Strategies:}
%\textcolor{red}{Ha} 
The whole training process spans $E$ epochs. 
%Each epoch has many batches $S_b$ with size $ms$ and each batch $S_b$ is a set of $m$ micro-batches $S_{b,h}$ with size $s$.
At the start of each epoch ${\tt Sample}_{s,m}$  generates sets $\{S_{b,h}\subseteq \{1,\ldots, N\}\}_{b=1,h=1}^{N/(ms),m}$ where each set $S_{b,h}$ has size $s$; we define $\{S_b=\bigcup_{h=1}^m S_{b,h}\}_{b=1}^{N/(ms)}$ where each set $S_b$ has size $ms$. Here, $b$ indexes the round within an epoch during which the client uses its training data to compute a local update that is transmitted to the server. After multiplying with the appropriate learning rates (step sizes $\eta_i$), the server aggregates received local updates from different clients into the global model maintained by the server. Within round $b$, $h$ indexes independent computations by an algorithm ${\cal A}$ (discussed later). Each computation starts from the client's local model. The $h$-th computation  is based on training data samples from data set $d$ that corresponds to $S_{b,h}$.  

In this paper we analyze and compare two distinct sampling strategies for ${\tt Sample}_{s,m}$:
\begin{itemize}
    \item {\bf Subsampling (SS):} Sets $S_b\subseteq \{1,\ldots, N\}$ with $|S_b|=ms$ are randomly sampled from $\{1,\ldots, N\}$. 
    \item {\bf Shuffling (SH):} The whole index set $\{1,\ldots, N\}$ is shuffled into a random order (according to a random chosen permutation). This is used to  partition data set $d$ into sets $S_b\subseteq \{1,\ldots, N\}$ with $|S_b|=ms$ in a random way. Notice that $d=\bigcup_{b=1}^{N/(ms)} S_b$.
\end{itemize}
The difference between the two strategies is that the $S_b$ are disjoint for shuffling while they may have intersections for subsampling. Once the $S_b$ are sampled,
%Next, for each $S_b$,  
${\tt Sample}_{s,m}$ selects a random chosen partition in order to split $S_b$ into subsets $S_{b,h}$, $1\leq h\leq m$, with $|S_{b,h}|=s$.

%Both subsampling and shuffling satisfy the following definition, which we will need in our general DP analysis as it turns out.

%\begin{ass}
%A sampling strategy
%\end{ass}


%\vspace{2mm}

\noindent 
{\bf Update Algorithm:}
%
%===========
%
% DONE -- see intro
%\textcolor{red}{Ha to Marten} The notation $w$ in algorithm $\mathcal{A}$ is quite confusing. As a reader, I think $w$ will not change in the for loop (lines 15 and 16). Therefore, I would assume $U$ resembles mini-batch SGD as we saw in the original paper of DP-SGD. Now, if I look at Algorithm 2, I can learn how we want to compute $a_h$, i.e., this is classical SGD. Therefore, based on line 17 of Algorithm 1 and Algorithm 2, I think the SGD here is something like we have $m$ threads and each thread we run classical SGD to compute one $a_h$. After all threads complete their tasks, we combine all computed grad $a_h$ in the fashion of mini-batch SGD. 
%
%I think you want to combine mini-batch SGD and classical SGD description here because this writing can allow you to talk batch clipping and individual clipping at the same time. If we have $m=1$ or we have only one thread, then the description is about classical SGD. If we have many threads and each thread has only one sample, i.e., the number of threads is equal to the number of datapoint in one batch, then we end up with mini-batch SGD. 
%
%Well, your main message is encrypted and it might be hard to see it. 
%
%Do you think we want to write your main message in a clear text? 
%
%[TO DO: I do think the current text is clear. But let;s put both Alg 1 and 2 in the intro with its detailed explanation here as is. In the intro we make a more intuitive explanation and clearly explain how the individual and batch clipping lead to two quite different sums which we will provide in the intro (and later refer to here).]
%
%=========
%
%
A round computes some partial update $a_h\leftarrow {\cal A}(w,\{\xi_i\}_{i\in S_{b,h}})$, 
%where $d=\{\xi_i\}_{i=1}^N$ and 
which only depends on $w$ and the set of training data samples $S_{b,h}$.
%During a round, $a_h\leftarrow {\cal A}(w,\{\xi_i\}_{i\in S_{b,h}})$, where $d=\{\xi_i\}_{i=1}^N$, computes some partial update $a_h$ which only depends on $w$ and the set of training data samples $S_{b,h}$. 
Here, $w$ is either equal to the most recent received global model or has been locally updated using some step size in combination with a local noised aggregated update $\bar{U}$ that was also transmitted to the central server. This means that any observer of communication with the central server is also able to compute the used $w$ based on previously observed updates $\bar{U}$. 

Algorithm ${\cal A}$ considers in sequence each of the $s$ training samples in $\{\xi_{i_1},\ldots, \xi_{i_s}\}$, where 
%$d=\{\xi_1, \ldots, \xi_N\}$ and 
$S_{b,h}=\{i_1,\ldots, i_s\}$ is the random index set produced by ${\tt Sample}_{s,m}$. 
%VVV %%%%%%%%%% REMOVE %%%%%%%%%%%%%
%For example,  ${\cal A}$ implements $s/v$ SGD iterations, where each iteration is based on an average gradient over a mini-batch of size $v$, see Algorithm \ref{alg:A}.
%
%\begin{algorithm}[H]
%\caption{Algorithm ${\cal A}$}
%\label{alg:A}
%\begin{algorithmic}[1]
%
%\State partition $S_{b,h}$ in sets $\{S_{b,h,j}\}_{j=1}^{s/v}$ of size $v$
%\State $w_1=w$
%\For{$j\in \{1,\ldots, s/v\}$}
%\State  $g_j= \frac{1}{v} \sum_{i\in S_{b,h,j}} \nabla f(w_j, \xi_{i})$ 
%\State $w_{j+1}=w_j - \eta_{(e-1)\frac{N}{ms}+b}\cdot g_j$
%\EndFor
%\State {\bf return} the aggregate update $a_h = \sum_{j=1}^{s/v} g_j$
%\State (notice that $w_{s/v+1}=w - \eta_{(e-1)\frac{N}{ms}+b}\cdot a_h$)
%\end{algorithmic}
%\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
We notice that our algorithmic framework and DP analysis allow any other optimization algorithm such as momentum based SGD. It may include batch normalization where normalization is done over the  batch $\{\xi_{i_1},\ldots, \xi_{i_s}\}$, and it may also include instance or layer normalization. 
We may even predefine a sequence of algorithms $\{{\cal A}_b\}_{b=1}^{N/(ms)}$ per epoch and use ${\cal A}_b$ in round $b$.
%(this allows inner plus outer loop type optimization algorithms \cite{Sarah, others?}). (\textcolor{red}{Ha to Marten: Do we really need to mention Sarah here? This is variance reduction method and it may be out of our scope because we need to compute many rounds with full gradient calculation.})
%may even have a sequence of round specific algorithms!]

%[APP] In practice we will also want to use data normalization as a pre-processing step. This requires computing the mean and variance over all data samples from $d$. This makes normalized data samples depend on all samples in $d$. For this reason we need differential private data normalization. That is, a differential private noisy mean and noisy variance is revealed a-priori. This leads to some privacy leakage. The advantage is that we can now re-write ${\cal A}$ as an algorithm that takes as input $w$, the original data samples $\{\xi_i\}_{i\in S_{b,h}}$ (as in our framework) together with the revealed noisy mean and noisy variance. ${\cal A}$ first normalizes each data sample after which it starts to compute gradients etc. In the $f$-DP framework, privacy leakage is now characterized as a trade-off function of the differential private data normalization pre-processing  composed with the trade-off function corresponding to our DP analysis for Algorithm \ref{alg:genDPSGD}.

%Our experiments uses SGD iterations where each $g_j$ is computed as an average over a mini-batch. That is, $S_{b,h}$ is split into a sequence of $s/v$ mini-batches, each of size $v$; $g_j=\frac{1}{v} \sum_{u=(j-1)v+1}^{jv} \nabla f(w_j,\xi_{i_u})$; and $1\leq j\leq s/v$.

%\vspace{2mm}

\noindent 
{\bf Clipping:}
To each computed  $a_h$ we apply clipping $x\rightarrow [x]_C=x/\max \{1, \|x\|/C\}$. We aggregate the clipped $[a_h]_C$ in a sum $U$. We add Gaussian noise before it is transmitted to the central server. Each round reveals one noisy update $U$ and we want to bound the aggregated differential privacy leakage. 
%
%
%
%VVV %%%%%%%%%% REMOVE
%For ${\cal A}$ defined in Algorithm \ref{alg:A}, the general formula for $U$ (before adding Gaussian noise) is
%============
%\begin{equation}
%U = \sum_{h=1}^m [\frac{1}{s} \sum_{i\in S_{b,h}} \nabla f(w,\xi_{i})]_C, \label{eq:gen}
%\end{equation}
%mini-batch and division by $m$ in line ... and at the server
%=============
%where $b$ is the round number (in the considered epoch) and $w_{h,j}$ denotes the computed $w_j$ in the $h$-th application of ${\cal A}$. Each application of ${\cal A}$ starts with $w_{h,1}=w$, the most recently received global model from the server (possibly updated with updates send to the central server, see lines 19 and 24 in Algorithm \ref{alg:genDPSGD}).
%We notice that $s=v=1$ corresponds to individual clipping  as given by (\ref{indclip}).
%At the other extreme, we may choose $m=1$ and $v=1$, which corresponds to batch clipping  (\ref{batchclip}). 
%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%Both (\ref{eq:gen})  and (\ref{batchclip})  are examples of the more general formulations
The general formula for $U$ is
\begin{equation}
    U=\sum_{h=1}^m [a_h]_C = \sum_{h=1}^m [{\cal A}(w,\{\xi_i\}_{i\in S_{b,h}})]_C.
    \label{eq:genA}
\end{equation}
%and, for $m=1$, 
%\begin{equation}
%    U= [{\cal A}(w,\{\xi_i\}_{i\in S_{b}})]_C.
%    \label{batchclipA}
%\end{equation}
%The latter is the general form of batch clipping for which our DP analysis of batch clipping in Table \ref{tab:DP} holds as well.
%%%%%%%%%%%%%%%%%%%%%%%


\noindent
{\bf Gaussian Noise:} After $U$ is computed according to (\ref{eq:genA}), Gaussian noise ${\cal N}(0,(2C\sigma)^2)$ is added to each entry of vector $U$. The resulting noisy update $\bar{U}$ after averaging by $m$ is sent to the central server.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% CLIPPING NOISE %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\vspace{2mm}
%
%\noindent
%{\bf Clipping Noise:} The clipping noise is defined as the difference between the clipped computations $U=\sum_{h=1}^m [a_h]_C$ and the originally intended non-clipped computations $\sum_{h=1}^m a_h$.
%We observe that as soon as convergence sets in, the computed gradients will start having smaller norms and as a result the clipping noise tends to zero. 
%
%Nevertheless, in order to start convergence, a large enough clipping constant $C$ is needed at the beginning. The disadvantage of a large $C$ is that the standard deviation of the added Gaussian noise per round becomes large and this hurts the accuracy of the final global model. The DP analysis will show to be general in that 
%we are allowed to adapt the used clipping constant at the start of each round. This can be used to reduce the added Gaussian noise per round once convergence sets in.
%
%During the initial phase where clipping noise is still prevalent, 
%the effect of $C$  with respect to individual clipping and batch clipping behaves differently:
%Let us first consider individual clipping (\ref{indclip}), i.e., formula (\ref{eq:gen}) with $s=v=1$. This shows a sum $U$ of $m$ clipped gradients, each clipped gradient having norm at most $C$. This implies that 
%$$\|U\|\leq mC,$$
%and, since clipping noise is not yet zeroed out during the initial phase, $\|U\|$ may be close to $mC$.
%Gaussian noise ${\cal N}(0,(2C\sigma)^2)$ is added to $U$. Relative to $U$'s norm the standard deviation of the added noise scales with $(2C\sigma)/(mC)=2\sigma/m$. 
%This may be a main reason  why individual clipping  start its convergence 
%despite the added noise (since for larger $m$ the relative noise gets smaller).
%
%On the other hand, batch clipping (\ref{batchclip}), i.e., formula (\ref{eq:gen}) with $m=v=1$ leads to a $U$ whose norm is 
%$$\|U\|\leq C.$$
%Again, since clipping noise is not yet zeroed out during the initial phase, $\|U\| \approx C$.
%Now, compared to individual clipping, the added Gaussian noise ${\cal N}(0,(2C\sigma)^2)$ is a factor $m$ larger relative to $U$'s norm; we have $2C\sigma/C=2\sigma$. This extra relative noise, compared to individual clipping, may lead to a slower start of convergence.
%
%We observe that once convergence sets in, the clipping noise gets close to zero and both $U=\sum_{h=1}^m [a_h]_C\approx \sum_{h=1}^m a_h$ for individual clipping and $U=[\sum_{h=1}^m a_h]_C\approx \sum_{h=1}^m a_h$ for batch clipping, where ${\cal A}$ implements its own mini-batch SGD (see introduction). Hence, both approaches will have the same added Gaussian noise relative to $U$'s norm. Therefore, both approaches enjoy a similar effect off the added Gaussian noise on convergence during the second phase after convergence has set in.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%may need to be compensated by choosing a larger parameter $m$ in (\ref{eq:gen}), rather than using a pure batch clipping approach with $m=1$. 

%by combininof a moving average. In the above notation, we want $\gamma$ to be a factor $m$ larger, where $m$ is used in individual clipping. This leads to a factor $m^2$ larger $a$ for the moving average.

%The above analysis is for when clipping noise occurs: If SGD starts to convergence, then the gradients will start having smaller norms and clipping is not applied and both individual clipping and batch clipping yield updates $U$ having the same or similar norms. This discussion shows that for future work simulation/experimental studies are needed to find the best parameter setting for the general formula (\ref{eq:gen}) and moving average with an update algorithm ${\cal A}$ (which may implement mini-batch clipping including averaging or not, or implement classical SGD, or an other SGD like algorithm). 




%\vspace{2mm}

\noindent
{\bf Some Remarks:} We notice that the framework allows a diminishing step size sequence (learning rate). The DP analysis shows that we may adapt the clipping constant at the start of each round. Rather than computing $U$ as the sum $\sum_{h=1}^m [a_h]_C$, we may compute $\sum_{h=1}^m {\cal B}([a_h]_{C'})$ for some post-processing function/procedure ${\cal B}$ (here, we need to take care that $\|{\cal B}(x)\|\leq C$ for $\|x\|\leq C'$). By revealing a differential private noisy mean and noisy variance of the training data set (due to differential private data normalization pre-processing), algorithm ${\cal A}$ can implement data normalization; in the $f$-DP framework, privacy leakage is now characterized as a trade-off function of the differential private data normalization pre-processing  composed with the trade-off function corresponding to our DP analysis for Algorithm \ref{alg:genDPSGD}. 
Without loss of differential privacy, we may under certain circumstances (by changing sampling to batches $S_b$ with non-fixed probabilistic sizes) use Gaussian noise ${\cal N}(0,(C\sigma)^2{\bf I})$, a factor $2$ less; a discussion is in Appendix \ref{app:factor}.

 
%... Gaussian noise starts DP ... explain the idea of a hypothesis; notice that subsampling/shuffling amplifies DP; still need composition .. see next section

\section{Background $f$-DP} \label{sec:GDPmain}

Dong et al. \citep{dong2021gaussian} introduced the state-of-the-art DP formulation based on hypothesis testing. From the attacker's perspective, it is natural to formulate the  problem of distinguishing two 
neighboring 
data sets $d$ and $d'$ based on the output of a DP mechanism ${\cal M}$ as a hypothesis testing problem:
$$\mbox{versus } \begin{array}{l}
H_0: \mbox{ the underlying data set is }d \\
H_1: \mbox{ the underlying data set is }d'.
\end{array}
$$
%$$ \mbox{ versus } \ \ \ \  H_1: \mbox{ the underlying data set is }d' .$$
Here, neighboring means that either $|d\setminus d'|=1$ or $|d'\setminus d|=1$. 
More precisely, in the context of mechanism ${\cal M}$, ${\cal M}(d)$ and ${\cal M}(d')$ take as input representations $r$ and $r'$ of data sets $d$ and $d'$ which are `neighbors.' The representations are mappings from a set of indices to data samples with the property that if $r(i)\in d\cap d'$ or $r'(i)\in d\cap d'$, then $r(i)=r'(i)$. This means that the mapping from indices to data samples in $d\cap d'$ is the same for the representation of $d$ and the representation of $d'$. In other words the mapping from indices to data samples for $d$ and $d'$ only differ for indices corresponding to the differentiating data samples in $(d\setminus d')\cup (d'\setminus d)$. In this sense the two mappings (data set representations) are neighbors.
In our main theorem we will consider the general case $g=\max\{ |d\setminus d'|, |d'\setminus d|\}$ in order to analyse `group privacy.' 

We define the Type I and Type II errors by
$$\alpha_\phi = \mathbb{E}_{o\sim {\cal M}(d)}[\phi(o)]  \mbox{ and } \beta_\phi = 1- \mathbb{E}_{o\sim {\cal M}(d')}[\phi(o)],
$$
where $\phi$ in $[0,1]$ denotes the rejection rule which takes the output of the DP mechanism as input. We flip a coin and reject the null hypothesis with probability $\phi$. The optimal trade-off between Type I and Type II errors is given by the trade-off function
$$ T({\cal M}(d),{\cal M}(d'))(\alpha) = \inf_\phi \{ \beta_\phi \ : \ \alpha_\phi \leq \alpha \},$$ 
for $\alpha \in [0,1]$, where the infimum is taken over all measurable rejection rules $\phi$. If the two hypothesis are fully indistinguishable, then this leads to the trade-off function $1-\alpha$. We say a function $f\in [0,1]\rightarrow [0,1]$ is a trade-off function if and only if it is convex, continuous, non-increasing, at least $0$, and $f(x)\leq 1-x$ for $x\in [0,1]$. 

We define a mechanism ${\cal M}$ to be $f$-DP if $f$ is a trade-off function and
$$
 T({\cal M}(d),{\cal M}(d')) \geq f
$$
for all neighboring $d$ and $d'$.
The $f$-DP framework supersedes all existing other frameworks in that a trade-off function contains all the information needed to derive known DP metrics such as $(\delta,\epsilon)$-DP and divergence based DPs. 
%Proposition 2.5 in \citep{dong2021gaussian} is an adaptation of a result in \citep{wasserman2010statistical} and states that a mechanism is $(\epsilon,\delta)$-DP if and only if the mechanism is $f_{\epsilon,\delta}$-DP, where
%$$f_{\epsilon,\delta}(\alpha) =
%\min \{ 0, 1-\delta - e^{\epsilon}\alpha, (1-\delta-\alpha)e^{-\epsilon}\}.
%$$
%We see that $f$-DP has the $(\epsilon,\delta)$-DP  formulation as a special case. It turns out that the original DP-SGD algorithm can be tightly analysed by using $f$-DP.

%\textcolor{red}{supersedes all other DP metrics, see their appendix and theorem for eps delta DP}

%\subsection{Gaussian DP}

%\vspace{2mm}
%
%\noindent
%{\bf Gaussian DP:}
%In order to proceed, 
\citep{dong2021gaussian} defines Gaussian DP as a special case of $f$-DP where $f$ is a trade-off function
$$G_\mu(\alpha) = T({\cal N}(0,1),{\cal N}(\mu,1))(\alpha) = \Phi( \Phi^{-1}(1-\alpha) - \mu )$$
with $\Phi$ the standard normal cumulative distribution of ${\cal N}(0,1)$. 
%We define a mechanism to be $\mu$-Gaussian DP if it is $G_\mu$-DP. Corollary 2.13 in \citep{dong2021gaussian} shows  that a mechanism is $\mu$-Gaussian DP if and only if it is $(\epsilon, \delta(\epsilon))$-DP for all $\epsilon\geq 0$, where
%\begin{equation} \delta(\epsilon) = \Phi(-\frac{\epsilon}{\mu}+\frac{\mu}{2}) - e^{\epsilon} \Phi(-\frac{\epsilon}{\mu}-\frac{\mu}{2}).
%\label{eq:gdp}
%\end{equation}

%%%%% SENSITIVITY %%%%%
%Suppose that a mechanism ${\cal M}(d)$ computes some function $u(d)\in \mathbb{R}^n$ and adds Gaussian noise ${\cal N}(0,(c\sigma)^2{\bf I})$; the mechanism outputs $o\sim u(d)+{\cal N}(0,(c\sigma)^2{\bf I})$. Suppose that $c$ denotes the sensitivity of function $u(\cdot)$, that is, $\|u(d)-u(d')\|\leq c$ for neighboring $d$ and $d'$ (the mechanism corresponding to one round update in Algorithm \ref{alg:genDPSGD} has sensitivity $c=2C$). After projecting the observed $o$  onto the line that connects $u(d)$ and $u(d')$ and after normalizing by dividing by $c$, we have that differentiating whether $o$ corresponds to $d$ or $d'$ is in the best case for the adversary (i.e., $\|u(d)-u(d')\|=c$) equivalent to differentiating whether a received output is from ${\cal N}(0,\sigma^2)$ or from  ${\cal N}(1,\sigma^2)$. Or, equivalently, from ${\cal N}(0,1)$ or from  ${\cal N}(1/\sigma,1)$. 
%This is how the Gaussian trade-off function $G_{\sigma^{-1}}$ comes into the picture. 

%\subsection{Subsampling}
%
%Besides implementing Gaussian noise, the original DP-SGD also uses random subsampling: For a data set $d$ of $N$ samples, ${\tt Sample}_m(d)$ (which in the notation of our general algorithmic framework corresponds to ${\tt Sample}_{s,m}(d)$ with $s=v=1$)  selects a subset of size $m$ from $d$ uniformly at random. We define convex combinations
%$$ f_p(\alpha) = p f(\alpha) + (1-p) (1-\alpha)$$
%with corresponding $p$-sampling operator 
%$$ C_p(f) = \min \{ f_p, f_p^{-1} \}^{**},
%$$
%where the conjugate $h^*$ of a function $h$ is defined as
%$$ h^*(y) = \sup_x \{ yx -h(x) \}$$ 
%and the inverse $h^{-1}$ of a trade-off function $h$ is defined as
%\begin{equation}
%h^{-1}(\alpha) = \inf\{t\in[0,1] \ | \ h(t)\leq \alpha \} \label{inverse}
%\end{equation}
%and is itself a trade-off function (as an example, we notice that $G_\mu=G_\mu^{-1}$ and we say $G_\mu$ is symmetric).
%Theorem 4.2 in \citep{dong2021gaussian} shows that if a mechanism ${\cal M}$ on data sets of size $N$ is $f$-DP, then the subsampled mechanism ${\cal M}\circ {\tt Sample}_{m}$ is $C_{m/N}(f)$-DP.


%The intuition behind operator $C_p$ is as follows. 
%First, ${\tt Sample}_m(d)$ samples the differentiating element between $d$ and $d'$ with probability $p$. In this case the computations ${\cal M}\circ {\tt Sample}_{m}(d)$ and  ${\cal M}\circ {\tt Sample}_{m}(d')$ are different and hypothesis testing is possible with trade-off function $f(\alpha)$. With probability $1-p$ no hypothesis testing is possible and we have trade-off function $1-\alpha$. This leads to the convex combination $f_p$. 

%Second, we notice that if $h=T({\cal M}(d),{\cal M}(d'))$, then $h^{-1}=T({\cal M}(d'),{\cal M}(d))$. Therefore, if ${\cal M}$ is $f$-DP (which holds for all pairs of neighboring data sets, in particular, for the pairs $(d,d')$ and $(d',d)$), then both $h\geq f$ and $h^{-1}\geq f$ and we have a symmetric upper bound $\min\{h,h^{-1}\}\geq f$. Since $f$ is a trade-off function, $f$ is convex and we can compute a tighter upper bound: $f$ is at most the largest convex function $\leq \min\{h,h^{-1}\}$, which is equal to the double conjugate $\min\{h,h^{-1}\}^{**}$. From this we obtain the definition of operator $C_p$.



%\subsection{Composition}

The tensor product $f\otimes h$ for trade-off functions $f=T(P,Q)$ and $h=T(P',Q')$ is well-defined by 
$$f\otimes h = T(P\times P',Q\times Q').$$
Let $y_i \leftarrow {\cal M}_i(\texttt{aux},d)$ with $\texttt{aux}=(y_1,\ldots, y_{i-1})$. Theorem 3.2 in \citep{dong2021gaussian} shows that if ${\cal M}_i(\texttt{aux},.)$ is $f_i$-DP for all $\texttt{aux}$, then the composed mechanism ${\cal M}$, which applies ${\cal M}_i$ in sequential order from $i=1$ to $i=T$, is 
$(f_1\otimes \ldots \otimes f_T)$-DP. The tensor product is commutative.
%$f^{\otimes T}$-DP.
%
As a special case Corollary 3.3 in \citep{dong2021gaussian} states that composition of multiple Gaussian operators $G_{\mu_i}$ results in $G_{\mu}$ where $\mu=\sqrt{\sum_i \mu_i^2}$.

%\subsection{Group Privacy}

%\vspace{2mm}
%
%\noindent
%{\bf Group Privacy:} 

Suppose that $d$ and $d'$ do not differ in just one sample, but differ in $g$ samples. \citep{dong2021gaussian} shows that if a mechanism is $G_\mu$-DP, then it is $G_{g\mu}$-DP for groups of size $g$. This shows a linear dependency in $g$.


%Theorem 2.14 in \citep{dong2021gaussian} analyzes how privacy degrades if $d$ and $d'$ do not differ in just one sample, but differ in $g$ samples. If a mechanism is $f$-DP, then it is $[1-(1-f)^{\circ g}]$-DP for groups of size $g$ (where $\circ g$ denotes the $g$-fold iterative composition of function $1-f$, where $1$ denotes the constant integer value $1$ and not the identity function, i.e., $(1-f)(\alpha)=1-f(\alpha)$). This is a tight statement in that {\em there exist} $f$ such that the trade-off function for groups of size $g$ cannot be bounded better. In particular, for $f=G_\mu$ we have $G_{g\mu}$-DP for groups of size $g$. This shows a linear dependency in $g$.


%rather than a multiplicative factor $g$ as in the mentioned $G_{g\mu}$-DP guarantee we show a $\sqrt{g}$ dependency. This is done by considering how, due to subsampling, the $g$ differentiating samples are distributed across all the rounds within an epoch and how composition of trade-off functions across rounds yields the $\sqrt{g}$ dependency.


A full description of $f$-DP (including the subsampling operator $C_{m/N}$) with intuitive explanation is in Appendix \ref{sec:GDP}.

%\subsection{Tight Analysis DP-SGD}
%
%We are now able to formulate the differential privacy guarantee of original DP-SGD 
%since it is a composition of  subsampled Gaussian DP mechanisms. Theorem 5.1 in \citep{dong2021gaussian} states that DP-SGD 
%as introduced in \cite{abadi2016deep} 
%is
%$$ C_{m/N}(G_{\sigma^{-1}})^{\otimes T}\mbox{-DP},$$
%where $T=(N/m)\cdot E$ is the total number of local rounds. 
%Since each of the theorems and results from \citep{dong2021gaussian} enumerated above are exact, we have a tight analysis.
%This leads in \citep{zhu2021optimal} to a (tight) differential privacy accountant (using a complex characteristic function based on taking the Fourier transform), which can be used by a client to understand when to stop  helping the server to learn a global model.


\section{DP Analysis}
\label{sec:DPanalysis}

%[TO DO: discuss max for g in appendix -- talk about $|d|=|d'|$ as formal requirement in appendix as is done in f-DP paper]

%[TO DO: move this as blueprint to the start of appendix C ... ; here we just explain that $\mathbb{P}$ yields $q_E(c)$ which sufficiently characterizes how differentiating samples are distributed over all the rounds ]

Our main theorems, stated below, are proved in Appendices \ref{sec:lemmas} and \ref{sec:DPproof}. We consider two data sets $d$ and $d'$ that differ in $g$ samples in order to also analyze group privacy. 

The main idea is to bound the sensitivity\footnote{The sensitivity of a value is the Euclidean norm between its evaluation for $d$ and $d'$ respectively.} of $\sum_{h=1}^m [a_h]_C$ in Algorithm \ref{alg:genDPSGD} by $2kC$ where $k$ is equal to the number of $a_h$ whose computation depends on differentiating samples (samples outside $d\cap d'$). The number of rounds $b$ within an epoch that have $k$ values $a_h$ that depend on differentiating samples is denoted by $c_k$. An epoch instance is into some extent characterized by the vector $(c_1,c_2,\ldots,c_g)$ where $c_k$ indicates the number of rounds that have sensitivity equal to $2kC$.

If a round has a sensitivity $2kC$, then the trade-off function of its corresponding mechanism, after adding Gaussian noise ${\cal N}(0,(2C\sigma)^2{\bf I})$, is given by the Gaussian trade-off function
%\footnote{We notice that our algorithmic framework can  have an a-priori selected diminishing sequence of  clipping constants per round as long as $\sigma$ remains fixed per round. A smaller clipping constant implies a smaller amount of added noise ${\cal N}(0,(2C\sigma)^2{\bf I})$ and this may help accuracy when gradients start to converge to zero. Since we normalize the Gaussian noise by dividing by the sensitivity, which scales linearly in the clipping constant, the Gaussian trade-off function and therefore our DP analysis remains the same.} 
$G_{k/\sigma}$. Therefore, an epoch instance $(c_1,c_2,\ldots,c_g)$ has a Gaussian trade-off function which is the composition of the round trade-off functions $G_{k/\sigma}$: We have
$$ 
G_{1/\sigma}^{\otimes c_1} \otimes G_{2/\sigma}^{\otimes c_2} \otimes \ldots \otimes G_{g/\sigma}^{\otimes c_g}= G_{\sqrt{\sum_{k=1}^g c_k k^2}/\sigma}.
$$
This can also be composed over multiple epochs.
This leads to defining a probability distribution $q_E(c)$ which is the probability that $E$ epoch instances together realize the value $c=\sqrt{\sum_{k=1}^g c_k k^2}$. 
%We can now conclude that the trade-off function of the overall mechanism ${\cal M}$ that describes Algorithm \ref{alg:genDPSGD} is 
%%equal to the expectation
%related to a sum 
%$\sum_c q_E(c)\cdot G_{c/\sigma}$. 
With probability $q_E(c)$, mechanism ${\cal M}$ executes a `sub-mechanism' which has trade-off function $G_{c/\sigma}$. The trade-off function of the overall mechanism ${\cal M}$ is therefore related, but not exactly equal, to the expectation $\sum_c q_E(c)\cdot G_{c/\sigma}$: See Lemma \ref{lem:mech1} in Appendix \ref{sec:lemmas}, we have
$T({\cal M}(d),{\cal M}(d'))\geq f$,  where $f(\alpha)$ equals the trade-off function
\begin{equation}  
%f(\alpha) = 
\inf_{\{\alpha_c\}} \left\{ \left. \sum_c q_E(c) G_{c/\sigma}(\alpha_c)  \ \right| \ \sum_i q_E(c) \alpha_c=\alpha \right\}. \label{eq:fsum}
\end{equation}
%is a trade-off function. 

Random variable $c_k$ counts the number of rounds within the $E$ epochs that have sensitivity $2kC$. The vector of random variables $(c_1,\ldots,c_g)$ defines the random variable $c=\sqrt{\sum_{k=1}^g c_k k^2}$. By analyzing its probability distribution $q_E(c)$ we are able to derive upper and lower bounds for $f$ defined in (\ref{eq:fsum}). The theorem provides a solution $f(\alpha)$ for the infinum and provides lower and upper bound functions. 
%
%==============
%
%\textcolor{red}{Ha to Marten} As I know, there is no paper having expectation $\sum_c q_E(c)\cdot G_{c/\sigma}$ when talking about the privacy. It might make audience confused. Actually, we want to explain $c_k$ is a random variable and thus, the vector $(c_1,\cdots,c_g)$ and $c$ are random variable. This explains why we derive the privacy curve is not $G_{c/\sigma}$ but $\sum_c q_E(c)\cdot G_{c/\sigma}$. It would be helpful for us when we are talking about the indv/batch clipping and subsampling/shuffling. 
%
%Actually, the representations of $E$ epochs and one epoch $e$ are the same, i.e., one vector $(c_1, \cdots, c_g)$ or one value $c$. Hopefully, the audience would not forget this fact. Otherwise, they might not be able to follow us. 
%
%It turns out that this sum should be regarded as a multi-variate function in variables $\alpha_c$, i.e., $\sum_c q_E(c)\cdot G_{c/\sigma}(\alpha_c)$, and we need to compute its infinum over all possible $\{\alpha_c\}$ such that $\sum_c q_E(c)\cdot \alpha_c=\alpha$. This infinum as a function of $\alpha$ is itself a trade-off function and is a lower bound for the trade-off function $T({\cal M}(d),{\cal M}(d')$ that we are interested in. The theorem provides a solution $f(\alpha)$ for the infinum and provides lower and upper bound functions. 
%
This leads to $T({\cal M}(d),{\cal M}(d') \geq f$ 
with upper and lower bounds which, see Table \ref{tab:DP}, can be very close to one another.
%%where $F$ can be further upper bounded and $f$ can be further lower bounded -- and we will see in next examples that these lower and upper bounds can be close to one another.
%We notice that DP analysis as done in the DP-SGD and $f$-DP papers \cite{abadi2016deep,dong2021gaussian} assumes the strong adversary as discussed in Section \ref{sec:GDP} who, translated to our general algorithmic framework, can  mimic/simulate computations $U=\sum_{h=1}^h [a_h]_C$ for the two hypothesis $d$ or $d'$ yielding $U$ or $U'$. After adding Gaussian noise this leads to the equivalent hypothesis testing of whether a sample is from $U+{\cal N}(0,(2C\sigma)^2)$ or $U'+{\cal N}(0,(2C\sigma)^2)$ and this gives the Gaussian trade-off function as discussed in Section \ref{sec:GDP} (where $\|U-U'\|\leq 2kC$). 
%%The next theorem is tight in that for this strong adversary $T({\cal M}(d),{\cal M}(d')\geq F$ can be met with equality. 

We first define/formalize a couple of concepts before stating our main theorems (proofs are in Appendices \ref{sec:lemmas} and \ref{sec:DPproof}).

%TO DO: put the first part in a definition; and the functions in another definition

\begin{definition} \label{def:qEc}
Let ${\cal M}$ be the mechanism  corresponding to our general framework for $E$ epochs which is based on ${\sf Sample}_{s,m}$ with $N$ equal to the size of the data set that is sampled. 
We require
%\footnote{This requirement only manifests itself in Appendix \ref{app:sampling}. Without this requirement, we need to define ${\cal C}$ and $q_E(c)$ using  sums $\sum_{k=1}^{m}$ rather than $\sum_{k=1}^g$ because all $\pi^e(S^e_{b,h})$ can have a non-empty intersection with $\{1,\ldots, g\}$. } 
that if ${\tt Sample}_{s,m}$ outputs $\{S^e_{b,h}\}_{b=1,h=1}^{N/(sm),m}$ for the $e$-th epoch, then for each $b$, $\{S^e_{b,h}\}_{h=1}^{m}$ partitions a set of size $ms$ into $m$ subsets $S^e_{b,h}$ of size $s$.
%
Define
$$ {\cal C} = \left\{ \sqrt{\sum_{k=1}^g c_k k^2} \ : \ \forall_k \ c_k\in \mathbb{N} \right\}.$$
The sampling procedure ${\tt Sample}_{s,m}$ defines a probability distribution $q_E(c)$ over ${\cal C}$ as follows (notice that $q_E(c)$ implicitly depends on $N$):
%[TO DO: fix appendix]
\begin{eqnarray*}
&& q_E(c) = \\
&& \hspace{-7mm} {\tt Pr}_{\{\pi^e\}}\left[ 
%\left. 
\begin{array}{c}
c^2=\sum_{k=1}^g 
%\# \{ (b,e) : L(\{\pi^e(S^e_{b,h})\}_{h=1}^m)=k\} \cdot 
c_kk^2 \\
\mbox{with } c_k=\# \{ (b,e) : L_{b,e}=k\} \mbox{ and}\\
 L_{b,e} = |\{ h \ : \ \pi^e(S^e_{b,h}) \cap \{1,\ldots, g\} \neq \emptyset \}| \\
\mbox{ conditioned on } \\
%\hspace{3cm} \ \left| \ 
\{ \{S^e_{b,h}\}_{b=1,h=1}^{N/(sm),m} \leftarrow {\tt Sample}_{s,m} \}_{e=1}^E 
%\right.
\end{array}
\right].
\end{eqnarray*}
%where
%$$
%L(\{\pi^e(S^e_{b,h})\}_{h=1}^m) = |\{ 1\leq h\leq m \ : \ \pi^e(S^e_{b,h}) \cap \{1,\ldots, g\} \neq \emptyset \}|.$$
\end{definition}

The next definitions define three trade-off functions based on $q_E(c)$ (which, as a consequence, also depend on $N$). The proof of the main theorems in Appendix \ref{sec:DPproof} show that the functions are well-defined.

\begin{definition} \label{def:f}
For distribution $q_E(c)$ over $c\in {\cal C}$ we define for $\alpha\in [0,1]$ function 
$$ f(\alpha)=\sum_{c\in {\cal C}} q_E(c) \cdot \Phi\left(\Lambda(\alpha)\cdot \frac{\sigma}{c} - \frac{c}{2\sigma}\right),$$
where function $\Lambda(\alpha)$, $\alpha\in [0,1]$, is implicitly defined by
    $$1-\alpha = \sum_{c\in {\cal C}} q_E(c) \cdot \Phi\left(\Lambda(\alpha)\cdot \frac{\sigma}{c} + \frac{c}{2\sigma}\right).$$
\end{definition}


\begin{definition}
Let $q_E(c)$ be a distribution over $c\in {\cal C}$. Let $u_{c^{\tt U}}$ and $c^{\tt U}$ be such that
$$
1\geq u_{c^{\tt U}} \geq \sum_{c\in {\cal C}: c<c^{\tt U}} q_E(c).
$$
Notice that $u_{c^{\tt U}}$ bounds the tail of $q_E(c)$ left from $c^{\tt U}$.

For $\alpha\in [0,1]$ we define  functions 
%$\hat{f}^{\tt U}_{c^{\tt U}}(\alpha)$ and $f^{\tt U}_{c^{\tt U}}(\alpha)$ as follows:
%For 
%$$
%1\geq u_{c^{\tt U}} \geq \sum_{c\in {\cal C}: c<c^{\tt U}} q_E(c)
%$$
%we define the functions
\begin{eqnarray*} \hat{f}^{\tt U}_{c^{\tt U}}(\alpha) &=& u_{c^{\tt U}}+(1-u_{c^{\tt U}})G_{c^{\tt U}/\sigma}(\alpha), \\
f^{\tt U}_{c^{\tt U}}(\alpha) &=& \min \{ \hat{f}^{\tt U}_{c^{\tt U}}, \hat{f}^{\tt U}_{c^{\tt U}}{}^{-1} \}^{**}(\alpha) \\
&=& 
\left\{
\begin{array}{ll}
u_{c^{\tt U}}+(1-u_{c^{\tt U}})G_{c^{\tt U}/\sigma}(\alpha),     &  \alpha \in [0,\beta_0], \\
\beta_0+\beta_1-\alpha,     &   \alpha\in [\beta_0,\beta_1], \\
G_{c^{\tt U}/\sigma}(\frac{\alpha -u_{c^{\tt U}} }{1-u_{c^{\tt U}}}),   &   \alpha \in [\beta_1,1],
\end{array}
\right.
\end{eqnarray*}
where
\begin{eqnarray*}
\beta_0 &=&
1- \Phi( \frac{c^{\tt U}}{2\sigma}-\frac{\sigma}{c^{\tt U}} \ln(1-u_{c^{\tt U}})), \\
\beta_1 &=& u_{c^{\tt U}} + (1-u_{c^{\tt U}})\cdot (1- \Phi(\frac{c^{\tt U}}{2\sigma}+\frac{\sigma}{c^{\tt U}} \ln(1-u_{c^{\tt U}}))).
\end{eqnarray*}
%For 
%$$
%u_{c^{\tt U}} = \sum_{c\in {\cal C}: c<c^{\tt U}} q(c)
%$$
%we define the function
%$$ f^{\tt U}_{c^{\tt U}}(\alpha)=u_{c^{\tt U}}+(1-u_{c^{\tt U}})G_{c^{\tt U}/\sigma}(\min \{1,\alpha/(1-u_{c^{\tt U}})\}),
%$$
%which is $\leq u_{c^{\tt U}}+(1-u_{c^{\tt U}})G_{c^{\tt U}/\sigma}(\alpha)$.
\end{definition}

\begin{definition}
Let $q_E(c)$ be a distribution over $c\in {\cal C}$. Let $l_{c^{\tt L}}$ and $c^{\tt L}$ be such that
$$
1\geq l_{c^{\tt L}} \geq \sum_{c\in {\cal C}: c>c^{\tt L}} q_E(c).
$$
Notice that $l_{c^{\tt L}}$ bounds the tail of $q_E(c)$ right from $c^{\tt L}$.

For $\alpha\in [0,1]$ we define  functions 
\begin{eqnarray*} \hat{f}^{\tt L}_{c^{\tt L}}(\alpha) &=& G_{c^{\tt L}/\sigma}(\min \{1,\alpha+l_{c^{\tt L}}\}), \\
f^{\tt L}_{c^{\tt L}}(\alpha) &=& \max \{ \hat{f}^{\tt L}_{c^{\tt L}}, \hat{f}^{\tt L}_{c^{\tt L}}{}^{-1} \}(\alpha) \\
&=& 
\left\{
\begin{array}{ll}
G_{c^{\tt L}/\sigma}(\alpha)-l_{c^{\tt L}},     &  \alpha\in [0,\beta],\\
G_{c^{\tt L}/\sigma}(\min \{1,\alpha+l_{c^{\tt L}}\}),     &  \alpha \in [\beta,1],
\end{array}
\right.
\end{eqnarray*}
where
$\beta\in [0,1]$ is implicitly defined as the (unique) solution of 
$$ G_{c^{\tt L}/\sigma}(\beta)-l_{c^{\tt L}} =\beta
$$
(and we notice that $\hat{f}^{\tt L}_{c^{\tt L}}{}^{-1}(\beta) = \beta = \hat{f}^{\tt L}_{c^{\tt L}}(\beta)$).
\end{definition}


\begin{theorem} \label{thm:main}
%
%TO DO all pairs $d$ and $d'$ with $g=\max \{ |d\setminus d'|, |d'\setminus d|\}$ and $N=|d\cap d'|+g$ (hence, $||d|-N|\leq g$, $||d'|-N|\leq g$, $||d|-|d'||\leq g$).
%
If ${\cal M}$ is $h$-DP for all pairs of data sets $d$ and $d'$ 
with $\max \{ |d\setminus d'|, |d'\setminus d|\}\leq g$ and $N=|d\cap d'|+g$,
%such that $\max\{ |d\setminus d'|, |d'\setminus d|\}\leq g$, 
then 
$$ h\leq f^{\tt U}_{c^{\tt U}} \leq \hat{f}^{\tt U}_{c^{\tt U}}$$
in adversarial model ${\cal A}_1$.
%(as explained in Section \ref{sec:GDP}).
%: repeat assumption, also discussion $N\neq N'$ -- do this separately.
We notice that $f^{\tt U}_{c^{\tt U}}$ is a symmetric trade-off function.
\end{theorem}

\begin{theorem} \label{thm:main2}
In adversarial model ${\cal A}_1$,
%(as explained in Section \ref{sec:GDP}) 
${\cal M}$ is $f$-DP for all pairs of data sets $d$ and $d'$ 
with $\max \{ |d\setminus d'|, |d'\setminus d|\}\leq g$ and $N=|d\cap d'|+g$. Trade-off function $f$ has  lower bound
$$ f\geq f^{\tt L}_{c^{\tt L}}\geq  \hat{f}^{\tt L}_{c^{\tt L}} .$$
Both $f$ and $f^{\tt L}_{c^{\tt L}}$ are symmetric trade-off functions.  For  larger $g$, $f$ becomes smaller (for all $\alpha$).  
%
%$f^{\tt L}_{c^{\tt L}}$ is a symmetric trade-off function
%=============
%The functions above depend on $N$. Remark: 
%
%Let $d$ and $d'$ with $N=|d|$ and $N'=|d'|$ and define $g=\max \{ |d\setminus d'|, |d'\setminus d|\}$, hence, $|N-N'|\leq g$. 
%and $d$ and $d'$ differ in at most $g$  samples.
%=============
%====================
%Then there exists a trade-off function $F$ such that
%$$ T({\cal M}(d),{\cal M}(d'))\geq F $$
%and
%$$ f^{\tt U}_{c^{\tt U}}\geq \hat{f}^{\tt U}_{c^{\tt U}} \geq F \geq f \geq f^{\tt L}_{c^{\tt L}}.
%$$
\end{theorem}

%\textcolor{red}{Ha to Marten} $q(c)$ is not defined anywhere before. I think you want to say $q_E(c)$. 



Notice that the adversary gets better in hypothesis testing when $f$ becomes smaller for larger $g$.
Therefore, in the worst case, the total number $t=|d\setminus d'|+|d'\setminus d|$ of samples in which $d$ and $d'$ differ are distributed as $|d\setminus d'|=t$ with $|d'\setminus d|=0$ (or vice versa) as this achieves the maximum value for $g$, i.e., $g=t$.

%=================

%I think you may want to tighten the upper bound by $min{f_u,f_u^-1}**$ trick
%because the $f_u$ is not symmetric. It is just a simple thing to make your
%result better.

%=========

%improve the upper bound $h=f^{{\sf U}}_{c^{{\sf U}}}$ to
%$$ \min \{ h, h^{-1} \}^{**}
%= \min \{\alpha \rightarrow u_{c^{\tt U}}+(1-u_{c^{\tt U}})G_{c^{\tt U}/\sigma}(\alpha), \alpha \rightarrow G_{c^{\tt U}/\sigma}(\frac{\alpha-u_{c^{\tt U}}}{1-u_{c^{\tt U}}}) \}^{**}.$$
%can we compute this precisely? does not matter -- just remark, also in lemma

%actually, for ease of readability, we already weakened the upper bound in the appendix ... 

%===========


%The bound $T({\cal M}(d),{\cal M}(d'))\geq F$ is tight under the standard adversarial model (see Appendix \ref{sec:DPproof} for explanation).

The difficulty of applying Theorems \ref{thm:main} and \ref{thm:main2} is in computing the probability distribution $q_E(c)$ -- the number of possible $c$ may be exponential in $g$ and $E$. Therefore, computing $f$ may be prohibited and only the lower and upper bound functions can possibly be estimated. Here, we remark that in general the lower and upper bounds are not tight together for small $E$; only for larger $E$ the probability distribution $q_E(c)$ will concentrate and   lower and upper bounds exist that  approach one another for large $E$.

%\section{Application of the General DP Theorems}

%[TO DO: just remove these bullet points and add small footnotes with some math in the intro where suitable]

In Appendices \ref{sec:subsampling} and \ref{sec:shuffling} we apply Theorems  \ref{thm:main} and \ref{thm:main2} to the DP analysis of subsampling and shuffling.  Table \ref{tab:DP} in the introduction summarizes the derived bounds\footnote{The table shows upper and lower bounds 
%can be constructed 
that are independent of $N$ or generally hold for large $N$ (as found in practice). Hence, the DP guarantees for ${\cal M}$ hold for all pairs of data sets $d$ and $d'$ 
with $\max \{ |d\setminus d'|, |d'\setminus d|\}\leq g$ (for the $g$ stated in the table). The condition $N=|d\cap d'|+g$ of the theorem can be discarded.}. 
%As  corollaries, this yields the contributions claimed in the introduction detailed below for the case where we do not use a moving average (this concept is introduced in the next section):
%\begin{itemize}
%    \item 
%We notice that applying our main theorems to individual clipping for general $g$ in order to find an upper bound on the trade-off function for mechanism ${\cal M}$ is left as an open problem. 

$\bullet$
%If 
%an upper bound can show that 
The stated lower bound $\approx G_{\sqrt{(e+\gamma)\min\{m,g\}gE}/\sigma}$ for individual clipping  is 
%tight, then the adversary is able to achieve the lower bound but cannot do better. 
%This expression is 
$\leq G_{\sqrt{gE}/\sigma}$, the trade-off function which the adversary can approximately achieve and cannot further improve for batch clipping. This shows that, unless the lower bound is not tight and can be improved upon,  batch clipping  provides a better DP guarantee since $G_{\sqrt{gE}/\sigma}$ is closer to the ideal trade-off function $1-\alpha$ (which corresponds to random guessing the hypothesis $d$ or $d'$).

%\item 
$\bullet$ Shuffling appears to concentrate $q_E(c)$ more compared to subsampling. This leads to sharper bounds: For the cases that can be compared, the ranges provided for subsampling prove  $G_{\sqrt{(1+1/\sqrt{2gE})gE}/\sigma}$-DP  while for shuffling we can prove  $G_{\sqrt{gE}/\sigma}$-DP which is closer to 
%$\alpha\rightarrow 
$1-\alpha$ since $G_{\sqrt{(1+1/\sqrt{2gE})gE}/\sigma}\leq G_{\sqrt{gE}/\sigma}$. Here, we note that $G_{\sqrt{gE}/\sigma}$ lies in the reported ranges for subsampling and with improved techniques it may be able to show that $G_{\sqrt{gE}/\sigma}$-DP is also true for subsampling. 
%However, 
For now, we can only show this for  large $E$ when $G_{\sqrt{(1+1/\sqrt{2gE})gE}/\sigma}$ tends to $G_{\sqrt{gE}/\sigma}$. 
%If $E$ is at most 50, then  this gives $G_{\sqrt{(1+1/\sqrt{2gE})gE}/\sigma}= G_{\sqrt{1.1\cdot gE}/\sigma}$, still relatively far from $G_{\sqrt{gE}/\sigma}$.



%\item 
$\bullet$
The table shows upper and lower bounds that are functions of the number $E$ of epochs, and are invariant with respect to the exact number of rounds per epoch. It turns out that even though more rounds lead to more updates that can be used for improved hypothesis testing, this is compensated for by each round update leaking less privacy due to the sampling  strategy (subsampling or shuffling).  So, we can freely choose the number of rounds in each epoch and this can be used to optimize for best accuracy.

%\item For the cases considered in the table, if $E\rightarrow \infty$ with $\sqrt{gE}/\sigma \rightarrow \mu$ for some $\mu>0$, then ${\cal M}$ tends to be $G_\mu$-DP. In particular, for individual clipping with subsampling and $g=1$ (the original DP-SGD), $C_{m/N}(G_{1/\sigma})^{\otimes (N/m)\cdot E}$-DP tends to $G_\mu$. 

%\item 
$\bullet$ The group privacy analysis using the $\circ$ operator in the original $f$-DP framework \cite{dong2021gaussian} based on our $g=1$ analysis gives a $G_{g\sqrt{E}/\sigma}$-DP like guarantee. This is not tight as our results show the much better tight $G_{\sqrt{gE}/\sigma}$-DP like dependency.
%\end{itemize}



%Independence rounds

%Asymptotic behavior shows  (general clipping (including individual clipping) with $g=1$; batch clipping with subsampling and $g\geq 1$; batch clipping with shuffling and $1\leq g\leq s$) ...

%We recognize a $\sqrt{g}$ rather than $g$ dependency -- so, the adversary has less info 


%For the analyzed cases, the theorem shows that shuffling does not weaken the DP guarantee that can be achieved by subsampling. For $g=1$, both achieve and cannot improve $\approx G_{\sqrt{E}/\sigma}$, and for batch clipping with $g\leq s$ both achieve and cannot improve $\approx G_{\sqrt{gE}/\sigma}$. 


%======================

%%%%%%%%% PHASES %%%%%%%%%%%%%%%%%
%We also notice that our theory can be used to analyze differential privacy for sampling based on parameters $s$ and $m$ that change from one epoch to the next; this allows one to implement a first phase where individual clipping is used to start convergence after with batch clipping is used to obtain better accuracy.
%%%%%%%%%%%%%%%%%%%%%%%
%while in addition shuffling allows us to have simple provable DP guarantees for group privacy.




%This shows into what extent the lower bound is tight.
%Lower bound $F\geq G_{\sqrt{gE}/\sigma}$ is tight for $g=1$ and also holds for $g>s$.



%, summarized below:
%    \begin{itemize}
%    \item We analyze general subsampling strategies. DP-SGD uses random subsampling. Another sampling strategy is shuffling which gives shuffling SGD. We show that both strategies (for either individual clipping or batch clipping) lead to approximately the same DP guarantees when neighboring data sets are considered. 
%    \item 

%    \item Our theory can be applied to analyzing group privacy leading to simple evaluable bounds.
%    %a non-closed formula for the DP guarantee). 
%    In particular, we show that group privacy for batch clipping scales with the square root of the size $g$ of the group, while group privacy for individual clipping has a worse dependence. This improves over the linear dependency of the size of the group in the current state-of-the-art $f$-DP framework. 
%    %We still have DP guarantees that scale with the square root of the total number of epochs.
    
%    \item We show that  DP guarantees (for both neighboring data sets and group privacy) scale with the square root of the total number $E$ of epochs, and is not dependent on the explicit number of rounds executed within these epochs. In other words, even though more local updates can be observed by the adversary, this turns out not to lead to more privacy leakage. This is because each local update is based on a smaller batch of training data samples which in itself leads to less privacy leakage per local update.
    %scales linearly in the group size.
%    \item We analyze the effect of data normalization on the DP guarantee.

%\item Precise results are listed in Table \ref{tab:DP} and discussed in Section \ref{sec:DPanalysis} where the above contributions are shown to be implied by the results in the table.
%\end{itemize}

==> Section_old/01_RelatedWork.tex <==
\section{Related Work}
\label{sec:01relatedwork}
{\color{red}TODO: add clipping methods in DPSGD papers}

{\color{red}TODO: add some privacy budget results from DPSGD papers}
% {\color{red}TODO: add different clipping methods in DPSGD papers}
{\color{red}TODO: add CIFAR10 comparisons table}


\begin{table}[H]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
 Method  & Model & Optimizer & $s$& $k$ &Test Accuracy & $(\epsilon,\delta)$ & BN layers\\ \hline
 DP-FTRL  & Convnet $(3C+2FC)$ & DP-FTRL & $2000$& $20$ & $70\%$ & $(20,1e-6 )$ & No\\ \hline
 Varun et al & Convnet $(2C + 2FC)$ & DPSGD & $64$ & $51$ & $ 51\%$ & $N/a$ &\\ \hline
 DPSGD(IC) & Convnet $(4C + 1FC)$  & DPSGD & $64$ & $50$ & $38.1\%$ & $( 0.5353, 1/50000)$ & No\\ \hline
 DPSGD(IC) & VGG16  & DPSGD & 2 & $50$ & 3& 4 & No\\ \hline
 DPSGD(BC) & Convnet $(4C + 1FC)$  & DPSGD & 2 & $50$ & 3& 4 & No\\ \hline
 DPSGD(BC + BN)  & Convnet & DPSGD & 2 & $50$ & 3& 4 & Yes\\ \hline
 DPSGD(BC)  & VGG16 & DPSGD & 2 & $50$& 3 & 4 & Yes\\ \hline
 DPSGD(BC + BN)  & VGG16 & DPSGD & 2 & $50$ & 3& 4 & Yes\\ \hline
\end{tabular}
\caption{Performance Comparison CIFAR10}
\label{table:Related_works}
\end{table}



==> Section_old/02_DPSGD_with_individual_clipping.tex <==
\section{DPSGD with Individual Clipping}
\label{subsec:02DPSGDwithIndividualClipping}

% \subsection{Differential Privacy w}
% \label{subsec:02differentialprivacy}
% {\color{red}TODO: Add Differential privacy definitions here}
Differential privacy \citep{dwork2006calibrating, dwork2011firm,dwork2014algorithmic,dwork2006our} defines privacy guarantees for algorithms on databases, in our case a client's sequence of mini-batch gradient computations on his/her training data set. The guarantee quantifies into what extent the output  of a client (the collection of updates communicated to the server) can be used to differentiate among two adjacent training data sets $d$ and $d'$ (i.e., where one set has one extra element compared to the other set).

\begin{defn} \label{defDP} A randomized mechanism ${\cal M}: D \rightarrow R$ is $(\epsilon, \delta)$-DP (Differentially Private) if for any adjacent $d$ and $d'$ in $D$ and for any subset $S\subseteq R$ of outputs,
$$ Pr[{\cal M}(d)\in S]\leq e^{\epsilon} Pr[{\cal M}(d')\in S] + \delta,$$
where the probabilities are taken over the coin flips of mechanism ${\cal M}$.
\end{defn}

The privacy loss incurred by observing $o$ is given by
$$ L^{o}_{{\cal M}(d) \| {\cal M}(d')} = \ln \left( \frac{Pr[{\cal M}(d)=o]}{Pr[{\cal M}(d')=o]} \right).
$$
As explained in \citep{dwork2014algorithmic} $(\epsilon, \delta)$-DP ensures that
for all adjacent $d$ and $d'$ the absolute value of privacy loss will be bounded by $\epsilon$ with probability at least $1-\delta$. 
The larger $\epsilon$ the more certain we are about which of $d$ or $d'$ caused observation $o$. 
When using differential privacy in machine learning we typically use $\delta=1/N$ (or $1/(10N)$) inversely proportional with the data set size $N$.

In order to prevent data leakage from  inference attacks in machine learning \citep{lyu2020threats} such as the deep leakage from gradients attack
\citep{ligengzhu201deepleakage,zhao2020idlg,geiping2020inverting} or the membership inference attack
\citep{shokri2017membership,nasr2019MIA,song2019MIA} a range of privacy-preserving methods have been proposed. 
Privacy-preserving solutions 
for federated learning are Local Differential Privacy (LDP) solutions \citep{abadi2016deep,abhishek2018privateFL,mohammad2020privateFL,stacey2018privateFL,meng2020privateFL,duchi2014local} and Central Differential Privacy (CDP) solutions \citep{mohammad2020privateFL,robin2017privateFL,mcmahan2017learning,nicolas2018privateFL,Yu2019CDP}. 
In LDP, the noise for achieving differential privacy is computed locally at each client and is added to the updates before sending to the server -- in this paper we also consider LDP. In CDP, a trusted server (aka trusted third party) aggregates received client updates into a global model; in order to achieve differential privacy the server adds noise to the global model before communicating it to the clients.  
\subsection{Deep Learning}
\label{subsec:02deeplearning}
{\color{red}TODO: Add Deep Learning models descriptions here}
\subsubsection{Image Classification}
\subsubsection{Shuffling Stocastic Gradient Descent}
\subsection{DPSGD}
{\color{red}TODO: Shows Abadi's individual clipping algorithm here}

==> Section_old/03_Differential_Privacy.tex <==
\section{Gaussian Differential Privacy}
\label{subsec:03GaussianDifferentialPrivacy}

==> Section_old/04_DPSGD_with_batch_clipping.tex <==
\section{DPSGD with Batch Clipping}
\label{sec:04DPSGDwithBatchClipping}


%%%% Shuffling Batch clipping algorithm %%%%%%
\begin{algorithm}[H]
\caption{Shuffling Batch Clipping DPSGD}
\label{alg:fed_batch_FL_DPs}
\begin{algorithmic}[1]
%\Procedure{LocalSGDwithDP}{$d,C,s,\sigma,T$}
\Procedure{Shuffling\_BatchClippingDPSGD}{}
    \State \textbf{Input:} dataset (D), batch size (s), number of epochs (K), learning rate ($\eta$), Gradient norm bound (C), noise scale $\sigma$, loss function L, model seed $\hat{w}_0$
    % \State N = len(D) \Comment{Get total number of rows in data set D}
    \State batches = divide\_dataset\_to\_batches(D,s) \Comment{detach dataset into equally data batches}
    \State B = len(batches)
    \For{batch \textbf{in} batches}
        \State normalize(batch) \Comment{Normalize data in each batch}
    \EndFor
    \For{k$= 0,1,2,\dots,K-1$}
        \State batches = shuffle(batches)
        \For{$b = 0,1,2,\dots, B-1$}
        \State $w=\hat{w}$
            \State U = 0
            \State batch = shuffle(batches[b])
            \For{$t = 0,1,\dots, s/m-1$}
                \State $g =\frac{1}{m} \sum_{i=0}^{m} \nabla L(w,batch[tm+i])$
                \State $w \leftarrow  w - \eta_{kB+b} \cdot g$
                \State $U \leftarrow U + g$
            \EndFor
            \State $U \leftarrow [U]_C$
            %$U/ \max(1,\frac{||U||_2}{C})$ 
            \Comment{Clipping gradient}
            \State $U\leftarrow U + N(0,C^2 \sigma^2 \textbf{I}) $ \Comment{Add noise to clipped gradients}
            \State $\hat{w} \leftarrow \hat{w} - \eta_{kB+b} \cdot U$
        \EndFor
    \EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}

[TO DO: explain leakage model of DPSGD and for us model $\hat{w}$ can be queried (not $w$)]

%%%% Shuffling individual clipping algorithm %%%%%%
\begin{algorithm}[H]
\caption{Shuffling Individual Clipping DPSGD}
\label{alg:fed_batch_FL_DPs}
\begin{algorithmic}[1]
%\Procedure{LocalSGDwithDP}{$d,C,s,\sigma,T$}
\Procedure{Shuffling\_IndividualClippingDPSGD}{}
    \State \textbf{Input:} dataset (D), batch size (s), number of epochs (K), learning rate ($\eta$), Gradient norm bound (C), noise scale $\sigma$, loss function L, model seed $\hat{w}_0$
    % \State N = len(D) \Comment{Get total number of rows in data set D}
    
%    \For{batch \textbf{in} batches}
%        \State normalize(batch) \Comment{Normalize data in each batch}
%    \EndFor
    \For{k$= 0,1,2,\dots,K-1$}
        \State D = shuffle(D)
        \State batches = divide\_dataset\_to\_batches(D,s) \Comment{detach dataset into equally data batches}
        \State B = len(batches)
 %       \State batches = shuffle(batches) ??? TO DO: shuffle over the whole data set, and then partition into batches, copy line 4 to here
        \For{$b = 0,1,2,\dots, B-1$}
        \State $w=\hat{w}$
            \State U = 0
            \State batch = batches[b] %shuffle(batches[b])
           \For{$t = 0,1,\dots, s-1$}
                \State $g =\nabla L(w,batch[t])$
                % \State $[g]_C = g/ \max(1)$
                \State $g\leftarrow [g]_C$
%                \State $w = w - \eta \cdot g$
                \State $U \leftarrow U + g$
            \EndFor
%            \State $U_c = U/ \max(1,\frac{||U||_2}{C})$ \Comment{Clipping gradient}
            \State $U \leftarrow U + N(0,C^2 \sigma^2 \textbf{I}) $ \Comment{Add noise to clipped gradients}
            \State $\hat{w} \leftarrow \hat{w} - \eta_{kB+b} \cdot U$
        \EndFor
    \EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}

[TO DO: explain how the original individial clipping is captures ($1/s$ into $\eta$)]

[TO DO: transfer of batch normalization from other publicized data set; or need DP version of batch normalization; or one does what we do]

[TO DO: what about the feature map based on PCA -- also this needs to be DP, or transferred]

[TO DO: ?? last theorem DPSGD paper -- what is meant by hyperparameters (topology of the model etc., or also PCA computations?)]
% \subsection{Masked Gradients}
% For the new masking algorithm, I am not that certain any more and somehow I cannot reproduce what I had in my mind. We should discuss. Right now I am thinking in the following confusing ways:

% We know from our Hogwild! analysis that we can partition the entries of a gradient vector in $D$ parts and select one of these at random -- and still yield 'optimal' convergence. For the selected part we keep the entries in the gradient. The non-selected parts are masked, that is, the entries in the gradient are set to zero.
 
% For strongly convex problems this leads to a factor $D$ slower convergence and this means we need $k'=kF$ epochs local gradient computations. The lower bound on $T$ is now a factor $D^2$ larger and this means a factor $D^2$ more rounds. This is fine if a solution for the sample size sequence exists: We recompute $\bar{s}'=\bar{s}/D$, hence, D can be at most $\bar{s}$.

% We used to clip the norm of the gradient down to $C$. But this is for all $D$ parts together. Each part can be seen to be separately clipped to $C' = C / \sqrt{D}$. And this is what will use for the masked gradient.

% Notice that $C'^2 (\sigma \sqrt{D}) ^2 = C^2 \sigma^2$. So, we keep the same noise as before. However, now the noise after renormalization with $C'$ yields a differential privacy noise of $\sigma*\sqrt{D}$. This gives a better (smaller) $\epsilon$. A huge improvement.

% We hope that the theory for strongly convex problems extrapolates to plain convex and non-convex problems.

% Rather than selecting one of $D$ parts at random, we can do better and only keep the part with the largest entries -- better convergence is expected. Or even better, we simply take the gradient and only keep the $D$ largest entries (in absolute values).

% There is one confusing aspect: We also know that the clipping constant cannot be arbitrarily reduced, hence, also $C'$ should be 'large enough'. By choosing a random part, we guarantee that our formula for $C'$ matches the effect of $C$ in the original distributed SGD algorithm, hence, if $C$ is large enough in the original setting, $C'$ will be large enough in this new masked setting. This argument shows that selecting a random part as strategy may be prefered.

% In the above analysis we push $D$ to $\bar{s}$ which makes $\bar{s}'=1$, that is, a single iteration. We also know that too small mini-batch or sample size does not work too well. Hence, we may only be able to use $D=\bar{s}/\text{large-enough-constant}$. A sensitivity study will help here.

% Notice that T meets our lower bound and this gives $\bar{s}=(N/k)/\text{const}$, that is, $\bar{s}'= (N/(Dk))/\text{const}$.

% The algorithm will work as follows:

% = We a-priori select a partition of vectors in $D$ parts.

% = We select one part at random and zero out the entries of the gradient in the other parts.

% = We clip the masked gradient by using clipping constant $C/\sqrt{D}$.

% = As before we add the masked-clipped gradients of the sample (mini-batch) together and add $N(0,C^2\sigma^2)$ noise. This will be the local round update $U$ with noise.


% \subsection{Diminishing Clipping constants}
% Main Goal: we want to have a decreasing sequence of clipping constants. We denote $M_i$ the decreasing sequence. $M_i$ has to be defined based on previous iterations, i.e., $0, 1,\dots, i-1$. We can use moving average to implement $M_i$.  

% Another really good idea in this line of thinking: Let $\bar{\eta}_i$ be the round step size.  We know we compute $s$ gradients in a single round. Suppose these gradients all have norm $n_i$. After aggregating the gradients, we see at most a norm $$\sqrt{s} \times n_i$$ and this is realized if all $s$ gradients sort of point into the ``same'' direction. We equate this to $$\bar{\eta}_i=\sqrt{s} \times n_i$$ and in this way we replace multiplying with the step-size by clipping with $n_i$. We still add the noise $$C\times \sigma \times \bar{\eta_i}$$ as before. This 
% implicitly includes multiplying with the step size $\bar{\eta}_i$. 
% We have $n_i=\bar{\eta}_i / \sqrt{s}$. The effective noise is now $$(C*\sigma*\bar\eta_i)/n_i = C*\sigma*\sqrt{s} = \sigma'.$$ This is very large. Notice that all of C is included and an extra $\sqrt{s}$ factor.

% Usually C is less than 1, say 0.1 or so. So, for this to work, we want $s>=100$.

% Now we always do clipping as this replaces multiplying with the step size. This also means we use the DP theory in a tight way (since this always pushes to the worst-case scenario for each data sample).

% Summarizing: We clip gradient with $$n_i=\bar\eta_i/\sqrt{s}$$ and we add noise $$\bar\sigma*\bar{\eta}_i$$ to the aggregated update at the end of the round. Here, $\bar{\sigma}$ plays the role of $C*\sigma$. And in our DP theory we use $$\sigma' = \bar{\sigma}*\sqrt{s}.$$


% % Toan comments

% DPSGD: $N(0, C^2 sigma^2 I)$
% this paper: $N(0, \bar{\sigma}^2)$

% $n_i = C'$: norm of 1 gradient.
% $new_sigma$ = $variance / n_1$
% $new_para = para + lr * (gradient + noise)$   

% 1. Standard format: $N(0,(C\sigma)^2)$ where $C\sigma$ is the variance of the noise and $C$ is the max norm of one gradient.  

% 2. At the $i$-th iteration, we have maximum norm of one gradient is $n_i$ or $C_i = n_i$. In this case, the aggregated norms is equal to $\sqrt{s}*n_i$ because we have $s$ gradients. The reason is very simple when we update the parameters, the information of $s$ gradients. Actually, $C_i = min(C,n_i)$.

% 3. Then I define $\bar{\eta}_i = \sqrt{s}*n_i$ and we can be sure that $n_i$ will get smaller by time. 

% We define stepsize $\bar{\eta}_i$ and from there, we can know $n_i$ or we can do reversely, compute $n_i$ and then we calculate $\bar{\eta}_i$

% 4. We say we want to create a new noise with variance $C\sigma \bar{\eta}_i$, then what is $C$ and $\sigma$ in this case? We may want to define $C = n_i$ because $n_i$ is the max norm of one gradient at the $i$-th iteration. From here, we already now noise variance:= $$C\sigma=n_i \sigma=C\sigma \bar{\eta}_i$$

% It means $\sigma$ or $\sigma' = C \sigma \sqrt{s}$. 

==> Section_old/05_BatchClipping_DP_Analysis.tex <==
\section{Batch Clipping DP Analysis}
\label{sec:05DPSGDbatchclippingDPanalysis}
{\color{red}TODO: This section shows how we build an accountant to compute the privacy budget $(\epsilon,\delta)$}

==> Section_old/06_Hyperparameters_configuration.tex <==
\section{Hyperparameters Configuration}
\label{sec:06hyperparametersconfiguration}

{\color{red}TODO: This section shows how we choose the hyperparameters in the experiments}

==> Section_old/07_Experiments.tex <==
\section{Experiments}
\label{sec:07experiments}



\begin{figure*}[th!]
\centering
%--------------SS, CIFAR10------------------%
\subfigure[CIFAR10,$SS$,$IC$]{\includegraphics[width=0.32\textwidth]{Section/Experiments/Individual_Clipping/Sum_gradient/convnet_subsampling_IC_lr_0.025_C_0.5_sigma_2_0.png}}
\subfigure[CIFAR10,$SS$,$BC$]{\includegraphics[width=0.32\textwidth]{Section/Experiments/Batch_Clipping/Sum_gradient/convnet_subsampling_BC_lr_0.025_C_0.01_sigma_2_0.png}}
\subfigure[CIFAR10,$SS$,$MC$]{\includegraphics[width=0.32\textwidth]{Section/Experiments/Mixing_clipping/Sum_gradient/convnet_subsampling_MC_lr_0.025_C_0.05_sigma_2_0.png}}\\
%--------------SF,CIFAR10------------------%
\subfigure[CIFAR10,$SH$,$IC$]{ \includegraphics[width=0.32\textwidth]{Section/Experiments/Individual_Clipping/Sum_gradient/convnet_shuffling_IC_lr_0.025_C_0.5_sigma_2_0.png}}
\subfigure[CIFAR10,$SH$,$BC$]{\includegraphics[width=0.32\textwidth]{Section/Experiments/Batch_Clipping/Sum_gradient/convnet_shuffling_BC_lr_0.025_C_0.01_sigma_2_0.png}}
\subfigure[CIFAR10,$SH$,$MC$]{\includegraphics[width=0.32\textwidth]{Section/Experiments/Mixing_clipping/Sum_gradient/convnet_shuffling_MC_lr_0.025_C_0.05_sigma_2_0.png}}\\
%----------------SS, MNIST----------------%
\subfigure[MNIST,$SS$,$IC$]{\includegraphics[width=0.32\textwidth]{Section/Experiments/Individual_Clipping/Sum_gradient/Lenet_subsampling_IC_lr_0.025_C_0.05_sigma_2_0.png}}
\subfigure[MNIST,$SS$,$BC$]{\includegraphics[width=0.32\textwidth]{Section/Experiments/Batch_Clipping/Sum_gradient/Lenet_subsampling_BC_lr_0.025_C_0.005_sigma_2_0.png}}
\subfigure[MNIST,$SS$,$MC$]{\includegraphics[width=0.32\textwidth]{Section/Experiments/Mixing_clipping/Sum_gradient/Lenet_subsampling_MC_lr_0.025_C_0.005_sigma_2_0.png}}\\
%-------------- SF, MNIST---------------%
\subfigure[MNIST,$SH$,$IC$]{\includegraphics[width=0.32\textwidth]{Section/Experiments/Individual_Clipping/Sum_gradient/Lenet_shuffling_IC_lr_0.025_C_0.005_sigma_2_0.png}}
\subfigure[MNIST,$SH$,$BC$]{\includegraphics[width=0.32\textwidth]{Section/Experiments/Batch_Clipping/Sum_gradient/Lenet_shuffling_BC_lr_0.025_C_0.005_sigma_2_0.png}}
\subfigure[MNIST,$SH$,$MC$]{\includegraphics[width=0.32\textwidth]{Section/Experiments/Mixing_clipping/Sum_gradient/Lenet_shuffling_MC_lr_0.025_C_0.005_sigma_2_0.png}}
\caption{CIFAR10 and MNIST testing accuracy for batch size $|S_b|= sm= 64,128,256,512,1028$ where $SS$ and $SH$ denote SubSampling and SHuffling, and where $IC$, $BC$ and $MC$ denote 
%SubSampling, ShuFfling, 
Individual Clipping ($s=1$), Batch Clipping ($m=1$) and Mixed Clipping, respectively. For MC, we set $s=64$ and $m=2,4,8$ and $16$. The used learning rate (step size) is $\mu=0.025$ (denoted by 'lr'), the used noise is given by $\sigma=2$ (denoted by 'sigma'), and the used clipping constant $C$ is fine-tuned for each separate setting. }
\label{fig:CIFAR10Accuracy}
\end{figure*}

In this section we provide a study on extending the mini-batch SGD approach of DP-SGD to include batch clipping as is allowed by the DP analysis of our general framework. We demonstrate that  Algorithm~\ref{alg:genDPSGD} can produce high accuracy models for different setups -- in our experiments, batch clipping yields accuracies comparable to DP-SGD with individual clipping, see Table \ref{tab:main_result}. 

\begin{table}[ht!]
\centering
\scalebox{0.8}{
\begin{tabular}{|c|c|c|c|}
\hline
 Sampling & Clipping  & CIFAR-10 & MNIST \\ \hline \hline
 $SS$& $IC$  & $71.09\% / 68.94\%$ & $98.41\% / 98.31\%$\\ \hline % Running
 $SS$& $BC$  & $71.7\% / 68.94\%$ & $98.21\% / 98.31\%$ \\ \hline %Done
 $SS$& $MC$ & $63.97\% / 68.94\%$  &    $97.5\% / 98.31\%$\\ \hline \hline %Done
 $SH$& $IC$ &  $70.77\% / 70.14\%$ & $98.38\% / 98.4\%$\\ \hline % Done
 $SH$& $BC$ & $71.52\% / 70.14\%$ & $98.33\% / 98.4\%$\\ \hline % Done
 $SH$& $MC$ & $64.68\% / 70.14\%$ & $96.97\% / 98.4\%$\\ \hline % Done
\end{tabular}
}
% TODO : rerun benchmark for shuffling SGD
%\caption{The best results of our proposed DP-SGD with different setups with CIFAR-10 and MNIST datasets, $\sigma$ = 2, learning rate $\eta = 0.025$ compared with classical SGD without DP where Subsampling, shuffling, individual clipping, batch clipping and mixing clipping are denoted as $SS, SH, IC,BC$ and $MC$, respectively.}
\caption{The best results among the different setups of Figure \ref{fig:CIFAR10Accuracy} for CIFAR-10 and MNIST with $\sigma=2$ and learning rate $\eta = 0.025$ compared to mini-batch SGD without DP.}
%where Subsampling, shuffling, individual clipping, batch clipping and mixing clipping are denoted as $SS, SH, IC,BC$ and $MC$, respectively.}
\label{tab:main_result}
\end{table}


Table \ref{tab:main_result} with Figure \ref{fig:CIFAR10Accuracy} depict accuracies for CIFAR-10~\cite{Krizhevskycifar10} and MNIST~\cite{lecun-mnisthandwrittendigit-2010} where we compute updates
\begin{equation}
U = \sum_{h=1}^m [\frac{1}{s} \sum_{i\in S_{b,h}} \nabla f(w,\xi_{i})]_C \label{eq:gen}
\end{equation}
with $s=1$ for Individual Clipping (IC) (this is DP-SGD), $m=1$ for pure Batch Clipping (BC), and values for $s$ and $m$ in between these two extremes denoted by Mixed Clipping (MC). We implement mini-batch SGD and therefore we use the same $w$ in our gradient computations in (\ref{eq:gen}).\footnote{Notice that division by $m$ is taken care of in lines 23 and 24 of Algorithm \ref{alg:genDPSGD} and division by $s$ is done in (\ref{eq:gen}) itself.} The initial learning rate (step size) is $\mu=0.025$ 
and, for each new epoch, the step size is decreased by a factor $\gamma=0.9$ if there is a decrease in testing accuracy between the last two consecutive epochs.
%
%with a decay rate of $\gamma = 0.9$ between consecutive epochs -- 
%we decrease the step size by $\gamma$ if there is a decrease in testing accuracy between two consecutive epochs
%from the current epoch to the next if the testing accuracy of the current epoch is lower \textcolor{red}{higher ??} than the testing accuracy of its previous epoch. 
%
In our settings we use the same $\sigma=2$ and compare experiments for each benchmark for the same  $E=100$ number of epochs gradient computations.

For each different setup, we report the best result among our grid-search in Table~\ref{tab:main_result}. For the image classification model of MNIST, we use LeNet-5 \cite{Lecun1998lenet5} which yields $98.31\%$ and $98.38\%$ testing accuracy for mini-batch SGD without DP for subsampling and shuffling. For our demonstration of being able to achieve similar high accuracy models, we use the lightweight Convolutional Neural Network (CNN) in Table \ref{tab:CIFAR10convNN} for CIFAR10. This has both fast training and good accuracy; $68.94\%$ and $70.14\%$ for mini-batch SGD without DP for subsampling and shuffling. 

\begin{table}[h]
\label{tab:CIFAR10convNN}
\centering
\scalebox{0.8}{
\begin{tabular}{|c|c|c|c|c|}
\hline
 Operation Layer & \#Filters  & Kernel size & Stride & Padding \\ \hline 
 \parbox[c]{3cm}{\vspace{1mm} \centering $Conv2D$+$ReLu$ \vspace{1mm}}& $32$ & $3 \times 3$ & $1 \times 1$ & $1 \times 1$\\ \hline 
 $AvgPool2d$& $1$  & $2 \times 2$ & $2 \times 2$ & $-$\\ \hline 
\parbox[c]{3cm}{\vspace{1mm} \centering $Conv2D$+$ReLu$\vspace{1mm}}& $64$ & $3 \times 3$ & $1 \times 1$ & $1 \times 1$\\ \hline 
 $AvgPool2d$& $1$  & $2 \times 2$ & $2 \times 2$ & $-$\\ \hline 
 \parbox[c]{3cm}{\vspace{1mm} \centering $Conv2D$+$ReLu$\vspace{1mm} }& $64$ & $3 \times 3$ & $1 \times 1$ & $1 \times 1$\\ \hline 
 $AvgPool2d$& $1$  & $2 \times 2$ & $2 \times 2$ & $-$\\ \hline 
 \parbox[c]{3cm}{\vspace{1mm} \centering $Conv2D$+$ReLu$ \vspace{1mm}}& $128$ & $3 \times 3$ & $1 \times 1$ & $1 \times 1$\\ \hline 
 $AdaptiveAvgPool2d$& $-$  & $-$ & $-$ & $-$\\ \hline 
 $Softmax$& $-$  & $-$ & $-$ & $-$\\ \hline 
\end{tabular}
}
\caption{CNN architecture for CIFAR-10 dataset}
\end{table}

This section reports an initial study and future work is needed to explore the more general algorithmic freedom in (algorithm ${\cal A}$ of) our framework for improving accuracy in specific application scenarios. As a result of our experiments, we can already conclude that for mini-batch SGD batch clipping is preferred over individual clipping because it allows being implemented with less memory overhead. This is because the implementation of (\ref{eq:gen}) with $m=1$ can keep track of just the gradient of the sum in the forward backward algorithm since $\sum_{i\in S_b} \nabla_w f(w,\xi_i) = \nabla_w \sum_{i\in S_b}  f(w,\xi_i)$,
%in (\ref{batchclip}) with TO DO, 
whereas mini-batch SGD with individual clipping needs to keep track of each of the gradients $\nabla_w f(w;\xi_i)$ since these need to be clipped before they can be summed together. 
This leads to a faster training process and smaller memory overhead compared to individual clipping, specifically, we trained the models using 11GB NVIDIA GTX1080ti GPUs with $15-30$ minutes running time for each batch clipping experiment and $4-6$ hours running time for each individual clipping experiment. 





%In this section, we demonstrate our experiments on DP-SGD with individual, batch and mixing clipping methods, with subsampling and shuffling methods (see Section~\ref{sec:alg}), and with CIFAR-10~\cite{Krizhevskycifar10} and MNIST~\cite{lecun-mnisthandwrittendigit-2010}. Since our main goal is showing Algorithm~\ref{alg:genDPSGD} can produce high accuracy model with different setups, all experiments have the same budget privacy (i.e., same $\sigma=2$ and number of epochs $E$), starting learning rate $\eta = 0.025$, learning rate decay rate $\gamma = 0.9$, image classification model, and the same algorithm $\mathcal{A}$ (i.e., it is mini-batch SGD andt the gradient $a_h$ is the mean of all gradients or 
%$U = \sum_{h=1}^m [a_h]_C = \sum_{h=1}^m [\frac{1}{|S_{b,h}|}\sum_{i\in S_{b,h}} \nabla f(w_{h},\xi_{i})]_C$). 

%============
%\begin{equation}
%U = \sum_{h=1}^m [\frac{1}{s} \sum_{i\in S_{b,h}} \nabla f(w,\xi_{i})]_C, \label{eq:gen}
%\end{equation}
%mini-batch and division by $m$ in line ... and at the server
%=============



%Besides, we only decrease the stepsize by $\gamma$ if there is a decrease in testing accuracy between two consecutive epochs. We note that finding high prediction accuracy algorithm $\mathcal{A}$ in the batch clipping mode is not our main research goal and we suggest it as a future work. 



%The results in Table~\ref{tab:main_result} shows that we can find a good candidate for each setup and all the results are not much different from each other. However, we observe that batch clipping based experiment can faster training process and smaller memory compared to individual clipping one because we do not need to save all clipped gradients as in individual clipping one.  Specifically, we trained the models using 11GB NVIDIA GTX1080ti GPUs with the running time is $15-30$ minutes for each batch clipping experiment and $4-6$ hours for each individual clipping experiments. 


% =============== TO DO ====

% [Toan's clipping? Formula (\ref{batchclipA}) (where $m=1$) with ${\cal A}$ executing mini-batch SGD without averaging (no division by $s$), this is discounted for in the round step size  :] As another example, ${\cal A}$ can also implement its own mini-batch SGD where all $w_j=w$ in (\ref{batchclip}); now, the clipping happens after summing the gradients of the mini-batch and this has the advantage of being implemented with less memory overhead compared to the mini-batch SGD with individual clipping. This is because the implementation can keep track of just the gradient of the sum in the forward backward algorithm since $\sum_{i\in S_b} \nabla_w f(w,\xi_i) = \nabla_w \sum_{i\in S_b}  f(w,\xi_i)$, whereas mini-batch SGD with individual clipping needs to keep track of each of the gradients $\nabla_w f(w;\xi_i)$ since these need to be clipped before they can be summed together. \textcolor{red}{TO DO: what can we show?} If we can show that mini-batch SGD with individual clipping (DP-SGD) compared to mini-batch SGD with batch clipping achieves a similar differential privacy guarantee and a similar accuracy of the final global model, then the latter will lead to the preferred implementation due to the much better memory utilization.

% =========================


%%%%%%%%% REWRITEN %%%%%%%%%%%
%We conduct a serial of experiments in order to analysis how good the Algorithm \ref{alg:genDPSGD} performs in many hyper-parameters settings. In Algorithm~\ref{alg:genDPSGD}, we run many communication rounds and in each communication we sample a batch $S_b$ which is partition into $m$ mini-batch $S_{b,h}, h=1,\dots,m$ with size $s$, i.e., $|S_{b,h}| = s$. We study batch clipping with $m=1$, individual clipping with $s=1$ and mixing clipping with $m>1$ and $s>1$. The experiment results are presented in Figure~\ref{fig:CIFAR10Accuracy}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Firstly, we have two main data sampling methods:
% \begin{itemize}
%     \item \textbf{Subsampling:}: We randomly sample each batch $S_b$ with batch size $|S_b| = ms $ from the dataset $\{1,2,...,N\}$. In this sampling method, a datapoint can re-appear in an epoch.
%     \item \textbf{Shuffling}: We divide the dataset $\{1,2,...,N\}$ into $N/ms$ batches with batch size $|S_b| = ms $. In this sampling method, every datapoint in the dataset appear only once in an epoch.
% \end{itemize}

% Secondly, Based on how we choose the $s$ and $m$ values, we run Algorithm \ref{alg:genDPSGD} in individual clipping or batch clipping manner:
% \begin{itemize}
%     \item If $m = 1$, then we have $U = \sum_{h=1}^m [a_h]_C = [a_1]_C$ where $a_1$ is the output computed from the batch $|S_b| = ms = s$. This leads to batch-clipping setting.
%     \item If $s = 1$, then we have $U = \sum_{h=1}^m [a_h]_C$ where $[a_h]_C$ is the output computed from a single datapoint. This leads to individual-clipping setting.
%     \item Moreover, our method also enables a new settings with mixed the effects of batch-clipping and individual-clipping by choosing $m > 1$ and $s > 1$.
% \end{itemize}

% Therefore, we run the experiments under the same hyper parameters except for the batch size $|S_b|=sm$ which is shown in Figure~\ref{fig:CIFAR10Accuracy}.




% \begin{figure*}[ht]
% \centering
% \subfigure[Subsampling,BC]{\includegraphics[width=0.32\textwidth]{Section/Experiments/Batch_Clipping/Sum_gradient/convnet_subsampling_BC_lr_0.025_C_0.01_sigma_2_0.png}}
% \subfigure[Subsampling,MC]{\includegraphics[width=0.32\textwidth]{Section/Experiments/Mixing_clipping/Sum_gradient/convnet_subsampling_MC_lr_0.025_C_0.05_sigma_2_0.png}}\\
% \subfigure[Shuffling,IC]{ \includegraphics[width=0.32\textwidth]{Section/Experiments/Individual_Clipping/Sum_gradient/convnet_shuffling_IC_lr_0.025_C_0.5_sigma_2_0.png}}
% \subfigure[Shuffling,BC]{\includegraphics[width=0.32\textwidth]{Section/Experiments/Batch_Clipping/Sum_gradient/convnet_shuffling_BC_lr_0.025_C_0.01_sigma_2_0.png}}
% \subfigure[Shuffling,MC]{\includegraphics[width=0.32\textwidth]{Section/Experiments/Mixing_clipping/Sum_gradient/convnet_shuffling_MC_lr_0.025_C_0.05_sigma_2_0.png}}
% \caption{CIFAR10 testing accuracy for batch size $|S_b| = sm = 64,128,256,512,1028$}
% \label{fig:CIFAR10Accuracy}
% \end{figure*}
%TODO: Add algorithm descriptions here
% To show the flexible of the algorithm ${\cal A}$,  we have several variations of algorithm ${\cal A}$ to see how the clipping step would affect the accuracy of the machine learning model:
% \begin{itemize}
% \item Case 1: The algorithm ${\cal A}$ outputs the sum of gradients of inputted batch.
% \item Case 2: The algorithm ${\cal A}$ outputs the average of gradients of the inputted data batch
% \end{itemize}
% Therefore, combining sampling methods with clipping settings, we have total 12 experiments with their best training accuracy and testing accuracy we achieved for CIFAR10 and MNIST dataset:
% \begin{table*}[]
% \centering
% \begin{tabular}{|c|c||c|c|}
% \hline
% \multicolumn{2}{|c||}{ CIFAR10 } & \multicolumn{2}{|c|}{MNIST} \\ \hline
%  (Sampling,Clipping)  & \parbox[t]{2.5cm}{Testing accuracy\\(DP/no-DP)}  &(Sampling,Clipping)  & \parbox[t]{2.5cm}{Testing accuracy\\(DP/no-DP)}  \\ \hline
%  Subsampling, IC  & $82.81\%$ & & $98.41\%$\\ \hline
%  Subsampling, BC  & $69.09\%$ & & $98.21\%$\\ \hline
%  Subsampling, MC &  & &   $97.5\%$\\ \hline
%  Shuffling,  IC&  $70.71\%$ & &$98.38\%$\\ \hline % Done
%  Shuffling ,  BC & $71.51\%$ & &$98.33\%$\\ \hline
%  Shuffling , MC &  & & $97.48\%$\\ \hline
% %  7&  $U = [\frac{1}{s}\sum_{h=1}^m a_h]_C + \frac{N(0,4C^2\sigma^2I)}{s}$& Subsampling & Batch clipping(s=1) & $73.42\%$ & $70.73\%$ \\ \hline
% %  8& $U = [\frac{1}{s}\sum_{h=1}^m a_h]_C + \frac{N(0,4C^2\sigma^2I)}{s}$& Subsampling & Batch Clipping(s=sm) & $72.998\%$ & $71.4\%$ \\ \hline
% %  9&  $U = [\frac{1}{s}\sum_{h=1}^m a_h]_C + \frac{N(0,4C^2\sigma^2I)}{s}$&Subsampling & Mixing &  & \\ \hline
% %  10&  $U = [\frac{1}{s}\sum_{h=1}^m a_h]_C + \frac{N(0,4C^2\sigma^2I)}{s}$&Shuffling &  Batch clipping(s=1)& $72.84\%$ & $70.91\%$\\ \hline
% %  11&  $U = [\frac{1}{s}\sum_{h=1}^m a_h]_C + \frac{N(0,4C^2\sigma^2I)}{s}$&Shuffling &  Batch Clipping(s=sm) & $74.03\%$  & $71.75\%$ \\ \hline
% %  12&  $U = [\frac{1}{s}\sum_{h=1}^m a_h]_C + \frac{N(0,4C^2\sigma^2I)}{s}$&Shuffling & Mixing &  & \\ \hline
% \end{tabular}
% \caption{CIFAR10 and MNIST dataset best testing accuracy (re running), $\sigma$ = 2, learning rate $\eta = 0.025$}
% \end{table*}
% Hyperparameters for setting 1: lr = 0.025, sm = 64, C = 0.5, sigma = 2
% Hyperparameters for setting 2: lr = 0.025, sm = 64, C = 0.005, sigma = 2
% Hyperparameters for setting 4: lr = 0.025, sm = 256, C = 0.5, sigma = 2
% Hyperparameters for setting 5: lr = 0.025, sm = 64, C = 0.01, sigma = 2
% Hyperparameters for setting 7: lr = 0.025, sm = 64, C = 0.5, sigma = 2
% Hyperparameters for setting 8: lr = 0.025, sm = 64, C = 0.01, sigma = 2
% Hyperparameters for setting 10: lr = 0.025, sm = 64, C = 0.5, sigma = 2
% Hyperparameters for setting 11: lr = 0.025, sm = 64, C = 0.01, sigma = 2
% \begin{table*}[t]
% \centering
% \begin{tabular}{|l|l|l|l|l|}
% \hline
%  Settings ID & Sampling method & Clipping Method & Training Accuracy & Testing accuracy  \\ \hline
%  1&   Subsampling & Toan batch clipping & $73.42\%$ & $70.73\%$ \\ \hline
%  2&  Subsampling & Batch Clipping & $72.998\%$ & $71.4\%$ \\ \hline
%  3&  Subsampling & Mixing &  & \\ \hline
%  4&  Shuffling &  Individual Clipping& $72.84\%$ & $70.91\%$\\ \hline
%  5&  Shuffling &  Batch Clipping & $74.03\%$  & $71.75\%$ \\ \hline
%  6&  Shuffling & Mixing &  & \\ \hline
% \end{tabular}
% \caption{CIFAR10 dataset training and testing accuracy with averaging gradients, $\sigma = 2$}
% \end{table*}
% Hyperparameters for setting 1: lr = 0.025, sm = 64, C = 0.5, sigma = 2
% Hyperparameters for setting 2: lr = 0.025, sm = 64, C = 0.01, sigma = 2
% Hyperparameters for setting 4: lr = 0.025, sm = 64, C = 0.5, sigma = 2
% Hyperparameters for setting 5: lr = 0.025, sm = 64, C = 0.01, sigma = 2
% \begin{table*}[t]
% \centering
% \begin{tabular}{|l|l|l|l|l|l|}
% \hline

% Settings ID & U formula & Sampling method & Clipping Method & Training Accuracy & Testing accuracy  \\ \hline
%  1&  $U = \frac{\sum_{h=1}^m [a_h]_C + N(0,4C^2\sigma^2I)}{s} $ &Subsampling &Individual Clipping & $98.41\%$ & $98.41\%$ \\ \hline
%  2&  $U = \frac{\sum_{h=1}^m [a_h]_C + N(0,4C^2\sigma^2I)}{s} $& Subsampling & Batch Clipping & $98.15\%$ & $98.21\%$\\ \hline
%  3&  $U = \frac{\sum_{h=1}^m [a_h]_C + N(0,4C^2\sigma^2I)}{s} $& Subsampling & Mixing & $97.55\%$ & $97.5\%$\\ \hline
%  4&  $U = \frac{\sum_{h=1}^m [a_h]_C + N(0,4C^2\sigma^2I)}{s} $&Shuffling &  Individual Clipping& $98.25\%$ & $98.38\%$\\ \hline
%  5&  $U = \frac{\sum_{h=1}^m [a_h]_C + N(0,4C^2\sigma^2I)}{s} $&Shuffling &  Batch Clipping & $98.13\%$& $98.33\%$ \\ \hline
%  6&  $U = \frac{\sum_{h=1}^m [a_h]_C + N(0,4C^2\sigma^2I)}{s} $&Shuffling & Mixing & $97.31\%$ & $97.48\%$\\ \hline
%  7& $U = \frac{\sum_{h=1}^m [a_h]_C + N(0,4C^2\sigma^2I)}{s} $&Subsampling & SGD &$98.26\%$ & $98.32\%$ \\ \hline
%  8& $U = \frac{\sum_{h=1}^m [a_h]_C + N(0,4C^2\sigma^2I)}{s} $&Shuffling & SGD & $98.29\%$& $98.4\%$\\ \hline
% %  9&  $U = [\frac{1}{s}\sum_{h=1}^m a_h]_C + \frac{N(0,4C^2\sigma^2I)}{s}$&Subsampling & Batch clipping (s=1)& $98.42\%$ & $98.41\%$ \\ \hline
% %  10&  $U = [\frac{1}{s}\sum_{h=1}^m a_h]_C + \frac{N(0,4C^2\sigma^2I)}{s}$&Subsampling & Batch Clipping (s=sm)& $98.14\%$ & $98.21\%$ \\ \hline
% %  11&  $U = [\frac{1}{s}\sum_{h=1}^m a_h]_C + \frac{N(0,4C^2\sigma^2I)}{s}$&Subsampling & Mixing &  & \\ \hline
% %  12&  $U = [\frac{1}{s}\sum_{h=1}^m a_h]_C + \frac{N(0,4C^2\sigma^2I)}{s}$&Shuffling & Batch clipping (s=1) & $98.25\%$ & $98.38\%$ \\ \hline
% %  13&  $U = [\frac{1}{s}\sum_{h=1}^m a_h]_C + \frac{N(0,4C^2\sigma^2I)}{s}$&Shuffling &  Batch Clipping (s=sm)& $98.15\%$& $98.35\%$ \\ \hline
% %  14& $U = [\frac{1}{s}\sum_{h=1}^m a_h]_C + \frac{N(0,4C^2\sigma^2I)}{s}$& Shuffling & Mixing &  & \\ \hline
%  15& Subsampling &$U = a_b$& SGD & $96.88\%$ & $98.34\%$\\ \hline
%  16& Shuffling & $U= a_b$&SGD &$98.44$\% &$98.38\%$ \\ \hline
% \end{tabular}
% \caption{MNIST dataset best training and testing accuracy, $\sigma$ = 2, learning rate $\eta = 0.025$}
% \end{table*}
% Hyperparameters for setting 1: lr = 0.025, sm = 64, C = 0.05, sigma = 2
% Hyperparameters for setting 2: lr = 0.025, sm = 64, C = 0.005, sigma = 2
% Hyperparameters for setting 3: lr = 0.025, sm = 128, s = 64, C = 0.005, sigma = 2
% Hyperparameters for setting 4: lr = 0.025, sm = 64, C = 0.005, sigma = 2
% Hyperparameters for setting 5: lr = 0.025, sm = 64,  C = 0.005, sigma = 2
% Hyperparameters for setting 6: lr = 0.025, sm = 128, s = 64, C = 0.005, sigma = 2
% Hyperparameters for setting 7: lr = 0.025, sm = 64
% Hyperparameters for setting 8: lr = 0.025, sm = 64
% Hyperparameters for setting 9: lr = 0.025, sm = 64, C = 0.05, sigma = 2
%Hyperparameters for setting 10: lr = 0.025, sm = 64, C = 0.005,sigma = 2, note: when C is too high (C> 0.5) the accuracy decrease significantly, acc <= 50%
%% Hyperparameters for setting 12: lr = 0.025, sm = 64, C = 0.5, sigma = 2
% Hyperparameters for setting 13: lr = 0.025, sm = 64, C = 0.005, sigma = 2
% Hyperparameters for setting 14: lr = 0.025, sm = 64, C = 0.005, sigma = 2
% Hyperparameters for setting 16: lr = 0.025, sm = 64
% Hyperparameters for setting 17: lr = 0.025, sm = 64

% \begin{table*}[t]
% \centering
% \begin{tabular}{|l|l|l|l|l|}
% \hline
%  Settings ID & Sampling method & Clipping Method & Training Accuracy & Testing accuracy  \\ \hline

%  1&  Subsampling & toan batch clipping (s=1)& $98.42\%$ & $98.41\%$ \\ \hline
%  2&  Subsampling & Batch Clipping (s=sm)& $98.14\%$ & $98.21\%$ \\ \hline
%  3&  Subsampling & Mixing &  & \\ \hline
% %  4&  Shuffling &  Individual Clipping& $\%$ & $\%$\\ \hline
%  5&  Shuffling & toan batch clipping (s=1) & $98.25\%$ & $98.38\%$ \\ \hline
%  6&  Shuffling &  Batch Clipping (s=sm)& $98.15\%$& $98.35\%$ \\ \hline
%  7&  Shuffling & Mixing &  & \\ \hline
%  8& Subsampling & SGD & $96.88\%$ & $98.34\%$\\ \hline
%  9& Shuffling & SGD &$98.44$\% &$98.38\%$ \\ \hline
% \end{tabular}
% \caption{MNIST dataset training and testing accuracy with averaging of sum of gradients, $U = [\frac{1}{s}\sum_{h=1}^m a_h]_C + \frac{N(0,4C^2\sigma^2I)}{s}$}
% \end{table*}

%TODO add figures (urgent, will do this tmr):

% Hyperparameters for setting 1: lr = 0.025, sm = 64, C = 0.05, sigma = 2
%Hyperparameters for setting 2: lr = 0.025, sm = 64, C = 0.005,sigma = 2, note: when C is too high (C> 0.5) the accuracy decrease significantly, acc <= 50%
%% Hyperparameters for setting 4: lr = 0.025, sm = 64, C = 0.5, sigma = 2
% Hyperparameters for setting 5: lr = 0.025, sm = 64, C = 0.005, sigma = 2
% Hyperparameters for setting 5: lr = 0.025, sm = 64, C = 0.005, sigma = 2
% Hyperparameters for setting 8: lr = 0.025, sm = 64
% Hyperparameters for setting 9: lr = 0.025, sm = 64

%============================================================FIGURES===========================%
% \begin{figure}[H]
% \centering

% \subfigure[Individual Clipping]{\includegraphics[width=0.49\textwidth]{Section/Experiments/Individual_Clipping/Sum_gradient/convnet_IC_lr_0.025_C_0.5_sigma_2_0.png}} 
% % \subfloat[setting 2]{\includegraphics[width=0.49\textwidth]{Experiments/DPSGD_acccuracy_graphs/SGD_DPSGD_comparison_setting_2.png}}\\
% % \subfloat[setting 3]{\includegraphics[width=0.49\textwidth]{Experiments/DPSGD_acccuracy_graphs/SGD_DPSGD_comparison_setting_3.png}} 
% % \subfloat[setting 4]{\includegraphics[width=0.49\textwidth]{Experiments/DPSGD_acccuracy_graphs/SGD_DPSGD_comparison_setting_4.png}} 

% \caption{CIFAR10 training accuracy and testing accuracy}
%     \label{fig:CIFAR10_accuracy}
 
% \end{figure}

% \begin{figure}[H]
% \centering

% \subfigure[Shuffling,Individual Clipping]{\includegraphics[width=0.49\textwidth]{Section/Experiments/Individual_Clipping/Sum_gradient/Lenet_IC_lr_0.025_C_0.5_sigma_2_0.png}} 
% \subfigure[Subsampling,Individual Clipping]{\includegraphics[width=0.49\textwidth]{Section/Experiments/Individual_Clipping/Sum_gradient/Lenet_subsampling_IC_lr_0.025_C_0.05_sigma_2_0.png}}\\
% \subfigure[Shuffling, Batch clipping]{\includegraphics[width=0.49\textwidth]{Section/Experiments/Batch_Clipping/Sum_gradient/Lenet_shuffling_BC_lr_0.025_C_0.005_sigma_2_0.png}} 
% \subfigure[Subsampling, Batch clipping]{\includegraphics[width=0.49\textwidth]{Section/Experiments/Batch_Clipping/Sum_gradient/Lenet_subsampling_BC_lr_0.025_C_0.005_sigma_2_0.png}} 

% \caption{MNIST training accuracy and testing accuracy}
%     \label{fig:MNIST_accuracy}
 
% \end{figure}
% {\color{red}TODO: Add privacy budget $(\epsilon,\delta)$ computed from privacy accountants}
% {\color{red}TODO: Add diminishing clipping experiments}


% We now have 4 experiments:


% CIFAR10 + DPA fixed sigma 
% TODO: Add figures for CIFAR10 SGD and DPSGD comparison in term of test accuracy

% \begin{figure}[H]
%     \centering
%     \includegraphics[scale=0.5]{Experiments/DPSGD_acccuracy_graphs/experiment_abadi_DPSGD_setting_1.png}
%     \caption{CIFAR10 accuracy test on Abadi DPSGD using setting 1}
%     \label{fig:experiment_abadi_DPSGD_setting_1}
% \end{figure}


% \begin{figure}[H]
% \centering

% \subfloat[setting 1]{\includegraphics[width=0.49\textwidth]{Experiments/DPSGD_acccuracy_graphs/SGD_DPSGD_comparison_setting_1.png}} 
% \subfloat[setting 2]{\includegraphics[width=0.49\textwidth]{Experiments/DPSGD_acccuracy_graphs/SGD_DPSGD_comparison_setting_2.png}}\\
% \subfloat[setting 3]{\includegraphics[width=0.49\textwidth]{Experiments/DPSGD_acccuracy_graphs/SGD_DPSGD_comparison_setting_3.png}} 
% \subfloat[setting 4]{\includegraphics[width=0.49\textwidth]{Experiments/DPSGD_acccuracy_graphs/SGD_DPSGD_comparison_setting_4.png}} 

% \caption{Test accuracy comparison between SGD and DPSGD under setting 1-4 for CIFAR10 dataset}
%     \label{fig:SGD_DPSGD_comparison_setting_1234}
%     % \label{fig:SGD_DPSGD_comparison_setting_1}
% \end{figure}

% \begin{figure}[H]
% \centering
% \subfloat[setting 5]{\includegraphics[width=0.49\textwidth]{Experiments/DPSGD_acccuracy_graphs/SGD_DPSGD_comparison_setting_5.png}} 
% \subfloat[setting 6]{\includegraphics[width=0.49\textwidth]{Experiments/DPSGD_acccuracy_graphs/SGD_DPSGD_comparison_setting_6.png}}\\
% \subfloat[setting 7]{\includegraphics[width=0.49\textwidth]{Experiments/DPSGD_acccuracy_graphs/SGD_DPSGD_comparison_setting_7.png}} 
% \subfloat[setting 8]{\includegraphics[width=0.49\textwidth]{Experiments/DPSGD_acccuracy_graphs/SGD_DPSGD_comparison_setting_8.png}} 
% \caption{Test accuracy comparison between SGD and DPSGD under setting 5-8 for CIFAR10 dataset}
%     \label{fig:SGD_DPSGD_comparison_setting_5678}
%     % \label{fig:SGD_DPSGD_comparison_setting_1}
% \end{figure}

% \begin{table}[H]
% \centering
% \begin{tabular}{|l|l|l|l|l|}
% \hline
%  Setting & 1,5 & 2,6 & 3,7 & 4,8\\ \hline
%  Our DPA (appendix) & 0.468 & 1.024 & 2.417 & 6.434 \\ \hline
%  Guassian DP accountant & 0.147 & 0.215 & 0.314 & 0.459 \\ \hline
%  Multiplication factor & 3.191 & 4.771 & 7.704 & 14.033 \\ \hline
% \end{tabular}
% \caption{Accountant (appendix) comparison  in terms of sigma given $\delta = 1/60000$ and  $\sigma = 10$ for CIFAR10 dataset}
% \label{table:accountant_comparison_appendix}
% \end{table}

% \begin{table}[H]
% \centering
% \begin{tabular}{|l|l|l|l|l|}
% \hline
%  Setting & 1,5 & 2,6 & 3,7 & 4,8\\ \hline
%  Our DPA (main body) & 0.225 & 0.225 & 0.225 & 0.225 \\ \hline
%  Guassian DP accountant & 0.147 & 0.215 & 0.314 & 0.459 \\ \hline
%  Multiplication factor & 1.531 & 1.047 & 0.716 & 0.490 \\ \hline
% \end{tabular}
% \caption{Accountant (main body) comparison in terms of sigma given $\delta = 1/60000$ and  $\sigma = 10$ for CIFAR10 dataset}
% \label{table:accountant_comparison_main_body}
% \end{table}


% \begin{figure}[H]
%     \centering
%     \includegraphics[scale=0.5]{Experiments/DPSGD_acccuracy_graphs/SGD_DPSGD_comparison_setting_2.png}
%     \caption{Test accuracy comparison between SGD and DPSGD under setting 2 for CIFAR10 dataset}
%     \label{fig:SGD_DPSGD_comparison_setting_1}
% \end{figure}
% \begin{figure}[H]
%     \centering
%     \includegraphics[scale=0.5]{Experiments/DPSGD_acccuracy_graphs/SGD_DPSGD_comparison_setting_3.png}
%     \caption{Test accuracy comparison between SGD and DPSGD under setting 3 for CIFAR10 dataset}
%     \label{fig:SGD_DPSGD_comparison_setting_1}
% \end{figure}

%TODO: ADD DPA fixed sigma:

% CIFAR10 + DPA with M-trick


% CIFAR10 + clipping with respect to the minimum of C and a moving average of previously computed gradient norms of prior rounds + DPA with M-trick

% CIFAR10 + clipping with $n_i=\bar{\eta_i}/\sqrt{s}$ and noise $\bar{\sigma}*\bar{\eta_i}$ and we do not multiply with $\bar{\eta_i}$ at the server side + DPA with M-trick         (here $\bar{\sigma}$ plays the role of $C*\sigma$ in the previous experiments -- but a sensitivity study can optimze $\bar{\sigma}$ independently)

% This starts to look like a great paper!!! (And we will write a separate one on the use of masking and this can be added to the above techniques.)



% Toan: This is the data for ICML rebuttal 
% %%% orifinal sigma %%%%
% \begin{table}[H]
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
%  s & 1 & 5 & 10 & 15 & 20 & 26\\ \hline
% Our DPA (appendix) & 0.0497 & 0.0497 & 0.0497 & 0.0497 & 0.0497 & 0.0497\\ \hline
% Guassian DP accountant & 0.0012 & 0.0037 & 0.0058 & 0.0075 & 0.0089 & 0.0105\\ \hline
% Multiplication factor & 42.3341 & 13.5508 & 8.6222 & 6.6648 & 5.5662 & 4.7309\\ \hline

% \end{tabular}
% \caption{Accountant (appendix) comparison (table 2) in terms of $\epsilon$ given $\delta = 1/10000$ and  $\sigma = 19.29962$ for LIBSVM dataset (N=10000), k = 5}
% \label{table:accountant_comparison_ICML_table_2}
% \end{table}

% \begin{table}[H]
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|l|}
% \hline
%  s & 10 & 25 & 50 & 100 & 200 & 300 & 370\\ \hline
% Our DPA (appendix) & 0.1521 & 0.1521 & 0.1521 & 0.1521 & 0.1521 & 0.1521 & 0.1521\\ \hline
% Guassian DP accountant & 0.0057 & 0.0097 & 0.0145 & 0.0215 & 0.0317 & 0.0398 & 0.0447\\ \hline
% Multiplication factor & 26.5983 & 15.6284 & 10.5079 & 7.0918 & 4.8017 & 3.8272 & 3.4047\\ \hline

% \end{tabular}
% \caption{Accountant (appendix) comparison (table 3) in terms of $\epsilon$ given $\delta = 1/60000$ and  $\sigma = 12.10881$ for MNIST dataset (N=60000), k = 6}
% \label{table:accountant_comparison_ICML_table_2}
% \end{table}

% \begin{table}[H]
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|l|}
% \hline
%  s & 10 & 25 & 50 & 100 & 300 & 500 & 689\\ \hline
% Our DPA (appendix) & 0.5253 & 0.5253 & 0.5253 & 0.5253 & 0.5253 & 0.5253 & 0.5253\\ \hline
% Guassian DP accountant & 0.0142 & 0.0239 & 0.0353 & 0.052 & 0.0957 & 0.127 & 0.1515\\ \hline
% Multiplication factor & 37.0619 & 22.0 & 14.8856 & 10.0999 & 5.487 & 4.1379 & 3.4676\\ \hline

% \end{tabular}
% \caption{Accountant (appendix) comparison (table 4) in terms of $\epsilon$ given $\delta = 1/50000$ and  $\sigma = 6.572$ for CIFAR10 dataset (N=50000), k = 7}
% \label{table:accountant_comparison_ICML_table_2}
% \end{table}
% %----%
% \begin{table}[H]
% \centering
% \begin{tabular}{|l|l|l|}
% \hline
%   & s\_min\_T = 26.066820  & s\_min\_T\_factor\_4 = 397.773976 \\ \hline
% Our DPA (main\_body) & 0.049700 & 0.049700 \\ \hline
% Guassian DP accountant & 0.010500 & 0.053300 \\ \hline
% Multiplication factor & 4.723400 & 0.932800 \\ \hline

% \end{tabular}
% \caption{Accountant (main body) comparison (table 2) in terms of $\epsilon$ given $\delta = 1/10000$ and  $\sigma = 19.29962$ for LIBSVM dataset (N=10000), k = 5}
% \label{table:accountant_comparison_ICML_table_2}
% \end{table}

% \begin{table}[H]
% \centering
% \begin{tabular}{|l|l|l|}
% \hline
%   & s\_min\_T = 288.099155  & s\_min\_T\_factor\_4 = 6085.935747 \\ \hline
% Our DPA (main\_body) & 0.152100 & 0.152100 \\ \hline
% Guassian DP accountant & 0.038900 & 0.209700 \\ \hline
% Multiplication factor & 3.914700 & 0.725700 \\ \hline

% \end{tabular}
% \caption{Accountant (main body) comparison (table 3) in terms of $\epsilon$ given $\delta = 1/60000$ and  $\sigma = 12.10881$ for MNIST dataset (N=60000), k = 6}
% \label{table:accountant_comparison_ICML_table_2}
% \end{table}

% \begin{table}[H]
% \centering
% \begin{tabular}{|l|l|l|}
% \hline
%   & s\_min\_T = 406.756279  & s\_min\_T\_factor\_4 = 15009.839116 \\ \hline
% Our DPA (main\_body) & 0.525300 & 0.525300 \\ \hline
% Guassian DP accountant & 0.113300 & 0.823900 \\ \hline
% Multiplication factor & 4.637200 & 0.637600 \\ \hline

% \end{tabular}
% \caption{Accountant (main body) comparison (table 4) in terms of $\epsilon$ given $\delta = 1/50000$ and  $\sigma = 6.572$ for CIFAR10 dataset (N=50000), k = 7}
% \label{table:accountant_comparison_ICML_table_2}
% \end{table}
% %%%% Double sigma %%%
% \begin{table}[H]
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
%  s & 1 & 5 & 10 & 15 & 20 & 26\\ \hline
% Our DPA (appendix) & 0.0124 & 0.0124 & 0.0133 & 0.0226 & 0.0336 & 0.0494\\ \hline
% Guassian DP accountant & 0.0003 & 0.0014 & 0.0023 & 0.003 & 0.0036 & 0.0043\\ \hline
% Multiplication factor & 35.7107 & 9.0472 & 5.9009 & 7.5678 & 9.2956 & 11.4712\\ \hline

% \end{tabular}
% \caption{Accountant (appendix) comparison (table 2) in terms of $\epsilon$ given $\delta = 1/10000$ and  $\sigma = 38.59924$ for LIBSVM dataset (N=10000), k = 5}
% \label{table:accountant_comparison_ICML_table_2}
% \end{table}

% \begin{table}[H]
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|l|}
% \hline
%  s & 10 & 25 & 50 & 100 & 200 & 300 & 370\\ \hline
% Our DPA (appendix) & 0.0376 & 0.0376 & 0.0376 & 0.0376 & 0.0695 & 0.1284 & 0.1799\\ \hline
% Guassian DP accountant & 0.0025 & 0.0043 & 0.0064 & 0.0095 & 0.0142 & 0.0179 & 0.0201\\ \hline
% Multiplication factor & 15.3177 & 8.8528 & 5.8925 & 3.9433 & 4.8945 & 7.1781 & 8.9323\\ \hline

% \end{tabular}
% \caption{Accountant (appendix) comparison (table 3) in terms of $\epsilon$ given $\delta = 1/60000$ and  $\sigma = 24.21762$ for MNIST dataset (N=60000), k = 6}
% \label{table:accountant_comparison_ICML_table_2}
% \end{table}

% \begin{table}[H]
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|l|}
% \hline
%  s & 10 & 25 & 50 & 100 & 300 & 500 & 689\\ \hline
% Our DPA (appendix) & 0.1267 & 0.1267 & 0.1267 & 0.1267 & 0.1487 & 0.3296 & 0.5686\\ \hline
% Guassian DP accountant & 0.0061 & 0.0104 & 0.0155 & 0.023 & 0.0427 & 0.0568 & 0.0679\\ \hline
% Multiplication factor & 20.7277 & 12.1549 & 8.1622 & 5.5028 & 3.4808 & 5.7994 & 8.3692\\ \hline

% \end{tabular}
% \caption{Accountant (appendix) comparison (table 4) in terms of $\epsilon$ given $\delta = 1/50000$ and  $\sigma = 13.144$ for CIFAR10 dataset (N=50000), k = 7}
% \label{table:accountant_comparison_ICML_table_2}
% \end{table}

% \begin{table}[H]
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
% \hline
%  s & 1 & 8 & 16 & 32 & 64 & 128 & 256 & 512 & 1024\\ \hline
% Our DPA (appendix) & 0.235 & 0.235 & 0.235 & 0.235 & 0.235 & 0.235 & 0.235 & 0.235 & 0.235\\ \hline
% Guassian DP accountant & 0.0013 & 0.0046 & 0.0069 & 0.0102 & 0.0151 & 0.0222 & 0.0327 & 0.048 & 0.0702\\ \hline
% Multiplication factor & 175.2506 & 51.0973 & 34.2703 & 23.0816 & 15.6017 & 10.5782 & 7.1911 & 4.8996 & 3.3447\\ \hline

% \end{tabular}
% \caption{Accountant (appendix) comparison in terms of $\epsilon$ given $\delta = 1/N$ and  $\sigma = 10$ for large dataset (N=100000), k = 5}
% \label{table:accountant_comparison_ICML_table_2}
% \end{table}

% \begin{table}[H]
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|}
% \hline
%  s & 1  & 16 & 32 & 64 & 128 & 256 & 512 & 1024\\ \hline
% Our DPA (appendix) & 0.2678 & 0.2678 & 0.2678 & 0.2678 & 0.2678 & 0.2678 & 0.2678 & 0.2678\\ \hline
% Guassian DP accountant & 0.0007 & 0.0034 & 0.005 & 0.0074 & 0.0108 & 0.0158 & 0.0231 & 0.0337\\ \hline
% Multiplication factor & 382.9444 & 78.4989 & 53.2876 & 36.2686 & 24.7421 & 16.9132 & 11.5822 & 7.944\\ \hline

% \end{tabular}
% \caption{Accountant (appendix) comparison in terms of $\epsilon$ given $\delta = 1/N$ and  $\sigma = 10$ for large dataset (N=500000), k = 5}
% \label{table:accountant_comparison_ICML_table_2}
% \end{table}
% %%% min_T experiments %%%%%%%%%%%%
% \begin{table}[H]
% \centering
% \begin{tabular}{|l|l|l|}
% \hline
%   & s\_min\_T = 8.7592  & s\_min\_T\_factor\_4 = 99.0425\\ \hline
% Our DPA (main\_body) & 0.0124 & 0.0124 \\ \hline
% Guassian DP accountant & 0.0021 & 0.0101 \\ \hline
% Multiplication factor & 6.0224 & 1.2299 \\ \hline

% \end{tabular}
% \caption{Accountant (main body) comparison (table 2) in terms of $\epsilon$ given $\delta = 1/10000$ and  $\sigma = 38.59924$ for LIBSVM dataset (N=10000), k = 5}
% \label{table:accountant_comparison_ICML_table_2}
% \end{table}

% \begin{table}[H]
% \centering
% \begin{tabular}{|l|l|l|}
% \hline
%   & s\_min\_T = 111.2648  & s\_min\_T\_factor\_4 = 1505.8654\\ \hline
% Our DPA (main\_body) & 0.0376 & 0.0376 \\ \hline
% Guassian DP accountant & 0.0102 & 0.0443 \\ \hline
% Multiplication factor & 3.7083 & 0.8503 \\ \hline

% \end{tabular}
% \caption{Accountant (main body) comparison (table 3) in terms of $\epsilon$ given $\delta = 1/60000$ and  $\sigma = 24.21762$ for MNIST dataset (N=60000), k = 6}
% \label{table:accountant_comparison_ICML_table_2}
% \end{table}

% \begin{table}[H]
% \centering
% \begin{tabular}{|l|l|l|}
% \hline
%   & s\_min\_T = 204.6154  & s\_min\_T\_factor\_4 = 3620.6131\\ \hline
% Our DPA (main\_body) & 0.1267 & 0.1267 \\ \hline
% Guassian DP accountant & 0.0345 & 0.17 \\ \hline
% Multiplication factor & 3.6748 & 0.7456 \\ \hline

% \end{tabular}
% \caption{Accountant (main body) comparison (table 4) in terms of $\epsilon$ given $\delta = 1/50000$ and  $\sigma = 13.144$ for CIFAR10 dataset (N=50000), k = 7}
% \label{table:accountant_comparison_ICML_table_2}
% \end{table}

% \begin{table}[H]
% \centering
% \begin{tabular}{|l|l|l|}
% \hline
%   & s\_min\_T = 612.6123  & s\_min\_T\_factor\_4 = 318796.613\\ \hline
% Our DPA (main\_body) & 0.235 & 0.235 \\ \hline
% Guassian DP accountant & 0.0529 & 0.3443 \\ \hline
% Multiplication factor & 4.4379 & 0.6824 \\ \hline

% \end{tabular}
% \caption{Accountant (main body) comparison in terms of $\epsilon$ given $\delta = 1/N$ and  $\sigma = 10$ for large dataset (N=100000), k = 5}
% \label{table:accountant_comparison_ICML_table_2}
% \end{table}

% \begin{table}[H]
% \centering
% \begin{tabular}{|l|l|l|}
% \hline
%   & s\_min\_T = 3098.1221  & s\_min\_T\_factor\_4 = 107121.3337\\ \hline
% Our DPA (main\_body) & 0.2678 & 0.2678 \\ \hline
% Guassian DP accountant & 0.0614 & 0.4127\\ \hline
% Multiplication factor & 4.3621 & 0.6489 \\ \hline

% \end{tabular}
% \caption{Accountant (main body) comparison in terms of $\epsilon$ given $\delta = 1/N$ and  $\sigma = 10$ for large dataset (N=500000), k = 5}
% \label{table:accountant_comparison_ICML_table_2}
% \end{table}

% \begin{table}[H]
% \centering
% \begin{tabular}{|l|l|l|}
% \hline
%   & s\_min\_T = 6213.1026  & s\_min\_T\_factor\_4 = 225559.356\\ \hline
% Our DPA (main\_body) & 0.2819 & 0.2819 \\ \hline
% Guassian DP accountant & 0.0647 & 0.4421\\ \hline
% Multiplication factor & 4.3553 & 0.6377 \\ \hline

% \end{tabular}
% \caption{Accountant (main body) comparison in terms of $\epsilon$ given $\delta = 1/N$ and  $\sigma = 10$ for large dataset (N=1000000), k = 5}
% \label{table:accountant_comparison_ICML_table_2}
% \end{table}


%%%% Skype Note from Marten %%%%%

% if accepted, we add a disclaimer: "due to the untimely death of Nhuong, we lost all his code. We realize that the lost code reported here use batch clipping instead. We notice that the accuracy improves if one uses individual clipping which allows a lower C for the same sigmas used in this paper. This means that the overall added Gaussian noise to a batch with individual clipping is much smaller compared to when batch clipping is used. For this reason we believe that the presented results also indicate what can at least be achieved when individial clipping is used, which is analysed in this paper.

% Add here: some evidence where you just create a simple comparison for your own CIFAR10 set up

% Add in the remark: Focus of the paper is the theoretical analysis ....

% Add that his code cannot be easily reconstructed as it implemented a full asynchronous FL solution, and this is now out of scope for us.

% Since we focus on the largest possible batch size (or minimal T) according to our theory

% Fixed sigma --- C\_batch and a C\_ind -- same k, T, s

% for a couple s and T combinations  (always fixed k=sT)


% ICML: disclaimer / extra C.3 section on experimental proof / C.4 extra about eps multiplication factor -- only report our best cases / how we can improve main body - intro, abstract, related work according to rebuttal

% 1) ind vs batch clipping

% 2) DPA plain vs DPA corrected for "sigma"

% 3) how to achieve best clipping: dynamic approach

% a) moving average

% b) from (2) we learn how to decrease clipping constant and this offers a proposal for a diminishing clipping constant sequence

% multiple benchmarks

% freedom around s and T



% \begin{figure*}[!ht]
% \begin{tabular}{ccccc}
%     \subfloat[IMS($RST_{0}$ vs org)]{\includegraphics[width=3cm,height=2cm]{Images/testBedIMPSa.pdf}\label{fig:RST0vsOrgIMS}} 
%    &\subfloat[CLKS($RST_{0}$ vs org)]{\includegraphics[width=3cm,height=2cm]{Images/testBedCLICKSa.pdf}\label{fig:RST0vsOrgCLKS}} 
%    &\subfloat[SPEND($RST_{0}$ vs org)]{\includegraphics[width=3cm,height=2cm]{Images/testBedSPENDa.pdf}\label{fig:RST0vsOrgSPEND}} 
%    &\subfloat[CTR($RST_{0}$ vs org)]{\includegraphics[width=3cm,height=2cm]{Images/testBedCTRa.pdf}\label{fig:RST0vsOrgCTR}}
%    &\subfloat[CPC($RST_{0}$ vs org)]{\includegraphics[width=3cm,height=2cm]{Images/testBedCPCa.pdf}\label{fig:RST0vsOrgCPC}} \\
%     \subfloat[IMS($RST_{750}$ vs $RST_{0}$)]{\includegraphics[width=3cm,height=2cm]{Images/750IMPS.pdf}\label{fig:750vsRST0IMS}} 
%    &\subfloat[CLKS($RST_{750}$ vs $RST_{0}$)]{\includegraphics[width=3cm,height=2cm]{Images/750CLICKS.pdf}\label{fig:750vsRST0CLKS}} 
%    &\subfloat[SPEND($RST_{750}$ vs $RST_{0}$)]{\includegraphics[width=3cm,height=2cm]{Images/750SPEND.pdf}\label{fig:750vsRST0SPEND}} 
%    &\subfloat[CTR($RST_{750}$ vs $RST_{0}$)]{\includegraphics[width=3cm,height=2cm]{Images/750CTR.pdf}\label{fig:750vsRST0CTR}}
%    &\subfloat[CPC($RST_{750}$ vs $RST_{0}$)]{\includegraphics[width=3cm,height=2cm]{Images/750ClearingPrice.pdf}\label{fig:750vsRST0CPC}} \\
%     \subfloat[IMS($Budget$ vs $RST_{0}$)]{\includegraphics[width=3cm,height=2cm]{Images/budgetIMPS.pdf}\label{fig:BUDGETvsRST0IMS}} 
%    &\subfloat[CLKS($Budget$ vs $RST_{0}$)]{\includegraphics[width=3cm,height=2cm]{Images/budgetCLICKS.pdf}\label{fig:BUDGETvsRST0CLKS}} 
%    &\subfloat[SPEND($Budget$ vs $RST_{0}$)]{\includegraphics[width=3cm,height=2cm]{Images/budgetSPEND.pdf}\label{fig:BUDGETvsRST0SPEND}} 
%    &\subfloat[CTR($Budget$ vs $RST_{0}$)]{\includegraphics[width=3cm,height=2cm]{Images/budgetCTR.pdf}\label{fig:BUDGETvsRST0CTR}}
%    &\subfloat[CPC($Budget$ vs $RST_{0}$)]{\includegraphics[width=3cm,height=2cm]{Images/budgetClearingPrice.pdf}\label{fig:BUDGETvsRST0CPC}} \\  
%     \subfloat[IMS($BudTime$ vs $RST_{0}$)]{\includegraphics[width=3cm,height=2cm]{Images/budgetTimeIMPS.pdf}\label{fig:BUDGETTIMEvsRST0IMS}} 
%    &\subfloat[CLKS($BudTime$ vs $RST_{0}$)]{\includegraphics[width=3cm,height=2cm]{Images/budgetTimeCLICKS.pdf}\label{fig:BUDGETTIMEvsRST0CLKS}} 
%    &\subfloat[SPEND($BudTime$ vs $RST_0$)]{\includegraphics[width=3cm,height=2cm]{Images/budgetTimeSPEND.pdf}\label{fig:BUDGETTIMEvsRST0SPEND}} 
%    &\subfloat[CTR($BudTime$ vs $RST_{0}$)]{\includegraphics[width=3cm,height=2cm]{Images/budgetTimeCTR.pdf}\label{fig:BUDGETTIMEvsRST0CTR}}
%    &\subfloat[CPC($BudTime$ vs $RST_{0}$)]{\includegraphics[width=3cm,height=2cm]{Images/budgetTimeClearingPrice.pdf}\label{fig:BUDGETTIMEvsRST0CPC}}
% \end{tabular}
% \caption{Comparison between 
% 1) The simulator/$RST_0$ (blue) vs Real system (orange) 
% 2) $RST_{750}$ (orange) vs $RST_0$ (blue)
% 3) $Budget$ (orange) vs $RST_0$ (blue) 
% 4) $Bud(get)Time$ (orange) vs $RST_0$ (blue)
% }\label{fig:manyComparison}
% \end{figure*}


% \begin{table*}[!ht]
% \centering
% \resizebox{\textwidth}{!}{%
% %\begin{center}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
%    \#campaigns   & 
%    \#campaigns w. active imp. interval Before & 
%    \#campaigns w. active imp. interval After &
%    \#campaigns w. positive lift& 
%    \#campaigns w. negative lift\\ \hline
%    56940 & 33602 & 33650 (+52) & 4362 (+13\%) & 7297 (+21.6\%) \\ \hline
%    \#campaigns   & 
%    \#campaigns w. active clk. interval Before & 
%    \#campaigns w. active clk. interval After &
%    \#campaigns w. positive lift& 
%    \#campaigns w. negative lift\\ \hline
%    56940 & 17913 & 18439 (+526) & 4466 (+24.22\%) & 7518 (+40.7\%) \\ \hline   
% \end{tabular}
% }
% \caption{\label{table:budgetRetention} Budget Retention Comparison between budgetTime and $RST_0$ pacing algorithms where $lift = 100\%(candidate - benchmark)/benchmark$ and $RST_0$ is benchmark}
% %\end{center}
% \end{table*}





==> Section_old/08_Conclusion.tex <==
\section{Conclusion}
\label{sec:08conclusion}

We have introduced a general algorithmic framework which allows strong $f$-DP guarantees in a slightly stronger adversarial model.
%can be proven based on a new proof technique. 
(a) The resulting DP guarantees have simple tight closed form formulas that are easily evaluated and interpreted (no DP accountant is needed), contrary to  existing $f$-DP guarantees (which use the more complex subsampling operator) in the adversarial model common in current literature. Existing $f$-DP guarantees have
%,  cited from \citep{dong2021gaussian}, 
"the disadvantage
that the expressions it yields are more unwieldy"
\citep{dong2021gaussian}.
%: they are computer evaluable, so usable in implementations, but do not admit simple closed form." 
(b) Our DP guarantees show invariance with respect to the number of rounds per epoch and show a $\sqrt{g}$
%, rather than $g$, 
dependency for group privacy. (c) Our general framework allows batch clipping together with a wide variety of optimization algorithms. 
%Initial experiments show that  batch-clipping in combination with mini-batch SGD yields comparable accuracy but with much better memory utilization leading to orders of magnitude faster training times. 
An open problem is whether advantages similar to (b) and (c) can be proven in the adversarial model common in current literature. And %for future work 
it also remains open into what extent the algorithmic freedom can be further exploited for improved accuracy and performance.


%, an improvement over the linear dependency in existing

%The $f$-DP guarantees come in simple to interpret formulas and 


 
%Finally, we introduce a fourth `moving average' DP principle next to adding Gaussian noise, sampling, and composition. It provides an additional extension to the general algorithmic framework and allows us, like subsampling, to significantly amplify DP and be able to exchange part of the DP amplification for a reduced clipping and Gaussian noise per update round. 

%\textcolor{red}{adversarial model, our table has lower bounds on what the weaker adversarial model would lead to -- no tight proofs yet available, open problem}

%    The resulting DP guarantees have simple closed form formulas that are easily evaluated, contrary to  existing $f$-DP guarantees which are based on the more complex subsampling operator and composition tensor. For the general $f$-DP theory,  cited from \citep{dong2021gaussian}, \textit{``the disadvantage
%is that the expressions it yields are more unwieldy: they are computer evaluable, so usable in
%implementations, but do not admit simple closed form."} We show that for the general algorithmic framework which includes the DP-SGD setting, we obtain simple and interpretable closed form characterizations.

%minibatch SGD with ind clipp vs general

%complex vs simple (no DP accountant needed, immeditate insight)

%linear g vs sqrt g (adoptable by A0)

%weaker adversary, better DP vs worse DP (but not too much!)
